A Survey on Traffic Signal Control Methods

Traffic signal control is an important and challenging real-world problem, which aims to minimize the travel time of vehicles by coordinating their movements at the road intersections. Current traffic signal control systems in use still rely heavily on oversimplified information and rule-based methods, although we now have richer data, more computing power and advanced methods to drive the development of intelligent transportation. With the growing interest in intelligent transportation using machine learning methods like reinforcement learning, this survey covers the widely acknowledged transportation approaches and a comprehensive list of recent literature on reinforcement for traffic signal control. We hope this survey can foster interdisciplinary research on this important topic.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> bk_RL.tex <==
% rlTLCS.tex

\section{Reinforcement Learning based Traffic Light Control}
\label{sec:rl-tlcs}
Recently, different artificial intelligent techniques have been proposed to control the traffic signal, like genetic algorithms~\cite{GoSr10}, swarm intelligence~\cite{Teod08}, and reinforcement learning~\cite{Wier00,MaDH16,KWBV08,ElAb12}. Among these technologies, RL is more effective and trending these years for online optimization without prior knowledge about the given environment. 



\nop{
Recently, different artificial intelligent techniques have been proposed to control the traffic signal, like genetic algorithms~\cite{GoSr10}, swarm intelligence~\cite{Teod08}, and reinforcement learning~\cite{wiering2000multi,mannion2016experimental,Kuyer2008,ElAb12}. Among these technologies, RL is more effective and trending these years for online optimization without prior knowledge about the given environment. Typically, these algorithms take the traffic as state,  signal operation as action, and learn from the rewards that the environment feedback. These studies vary in four folds as follows: 
(1) \emph{RL method}. Earlier methods use tabular Q-learning \cite{APK03,ElAb10} to learn the value function which requires the state to be discrete thus cannot scale up to a large state space for complicated scenarios in traffic signal control. To solve this problem, recent studies propose to apply Deep Q-learning~\cite{wei2018intellilight} or policy gradient methods~\cite{mousavi2017traffic} using continuous state representations. 
(2) \emph{Reward Design}. Previous studies consider different factors in reward function design including including average delay~\cite{ALUK10,drl}, 
average travel time~\cite{liu2017cooperative}, 
and queue length~\cite{wei2018intellilight,liLW16}.
(3) \emph{State Design}. State representation typically include queue length~\cite{wei2018intellilight,liLW16}, average delay~\cite{GenR16,drl}, and image features~\cite{gao2017adaptive, liu2017cooperative,drl}. 
(4) \emph{Coordination}. Coordination could benefit the signal control for multi-intersection scenarios. Explicit coordination strategies include manually adjust offsets~\cite{urbanik2015signal}, coordination graphs~\cite{KWBV08,VaOl16}, hierarchical multi-agent RL ~\cite{YCTS05,FrGh03}, or simply using a central agent to control all the intersections~\cite{brockfeld2001optimizing}. 
}
\subsection{Preliminaries}


% \begin{table}[htb]
%   \caption{Notations}
%   \label{tab:notations}
%   \begin{tabular}{ll}
%     \toprule
%     Notation&Meaning\\
%     \midrule
%     $\environment$   & Environment                 \\
%   	$\agent$         & Agent                       \\
%     $\action$        & Action                      \\
%     $\staterep$      & State                       \\
%     $\reward$        & Reward                      \\
%     $\qnetwork$      & \deepQNetwork                   \\
%     $\queueLength_\laneIndex $ & Queue length on lane $\laneIndex$ \\
% 	$\numOfVehicles_\laneIndex $ & Number of vehicles on lane $\laneIndex$ \\
% 	$\averageWaitingTime_\laneIndex $ & Average waiting time of vehicles on lane $\laneIndex$ \\
% 	$\image \in \mathbb{R}^{N \times N}$ & Image representation of vehicles' position \\
% 	$\phase_c $ & Current phase \\
% 	$\phase_n $ & Next phase \\
% 	$\switch \in \left\{0,1\right\}$  & Light switches (1) or not (0) \\
%     $\delay_\vehicleIndex $ & Delay of vehicle $\vehicleIndex$. \\
% 	$\emergencyStop_\vehicleIndex$ & Number of emergency stops of vehicle $\vehicleIndex$. \\
    
%   \bottomrule
% \end{tabular}
% \end{table}
\subsubsection{Basic concepts}

In order to solve the traffic signal control problem using RL, we first introduce the formulation of RL in Problem~\ref{pro:RLI}, then we introduce how traffic signal control fits the RL setting.

\begin{problem}[RL Framework] 
\label{prob:RLI}
Usually a single-agent RL problem is modeled as a Markov Decision Process (MDP) $<\mathcal{S}, \mathcal{A}, P, \mathcal{R}, \gamma>$, which models an agent interacting with environment at discrete time steps $t$. It has a set of states, $\mathcal{S}$, a set of actions $\mathcal{A}$, environment reward function 
$\mathcal{R}$ that determines the reward $\reward$ as :$\mathcal{S}\times\mathcal{A}\times\mathcal{S}\rightarrow\mathbb{R}$ 
and a probabilistic state transition function 
$P:\mathcal{S}\times\mathcal{A}\times\mathcal{S}\rightarrow[0,1]$. 
At time step t, the agent observes state $s_t\in\mathcal{S}$ and takes action $a_t\in\mathcal{A}$. The agent observes the next state $s_{t+1}$, drawn
from the transition probability distribution $P(s_t, a_t,\cdot)$, and a reward $r_t = R_{env}(s_t, a_t, s_{t+1})$. The behavior is defined by a policy 
$\pi: \mathcal{S}\times\mathcal{A}\rightarrow[0,1]$, 
which represents the selection probabilities over
actions. The goal of an agent is to find a policy that maximizes the expectation of the return, which is the discounted sum of rewards: $G_t := \sum_{i=0}^\infty\gamma^i r_{t+i}$
, where the discount factor $\gamma \in [0, 1]$ controls the importance of immediate rewards versus future rewards. Each policy $\pi$ has a corresponding action-value function that gives the expected return conditioned on the state and action, when acting according to that policy: $ Q^\pi(s,a) = \mathbb{E}[G_t|s_t=s,a_t=a,\pi]
$

The optimal policy $\pi^*$ can be found by iteratively improving an estimate of the optimal action-value function $Q^*(s, a) := \max_\pi Q^\pi(s, a)$, using sample-based updates. Once $Q^*$
is sufficiently approximated, acting greedy with respect to it yields the optimal policy.

The Q-value function is commonly estimated using a function approximator with weight vector $\theta: Q(s, a; \theta)$. Deep Q-Network (DQN) uses a deep neural network as function approximator and iteratively improves an estimate of $Q^*$ by minimizing the sequence of loss functions, where $i$ stands for the $i$-th iteration:

\begin{subequations}
\begin{align}
\label{eq:loss}
\mathcal{L}_i(\theta_i) = \mathbb{E}_{s,a,r,s'}[(y_i^{DQN}-Q(s,a;\theta_i))^2]\\
y_i^{DQN}=r+\gamma\max_{a'}Q(s',a';\theta_{i-1})
\end{align}
\end{subequations}


For a single intersection, the goal of a traffic signal agent $\agent$ controlled with RL is to learn the optimal action value function $Q^*(s,a)$. At every time step $t$, $\agent$ observes from its environment $\environment$, takes action $\action_t$ that maximize the reward $r_t$ (i.e., the performance of the intersection), given the state $\staterep_t$ (describing the positions of vehicles near this intersection).

\end{problem}

\begin{problem}[Multiagent RL Framework]
Learning in systems with multiple players has a long history in game theory. The generalization of a MDP for $n$ agents is a Stochastic Game (SG), represented by the tuple $<\agentVec, \pmb{S}, \pmb{A}, \mathcal{R}, \pmb{P}>$, where $\pmb{G}$ is a set of agents, $\pmb{S}=\times S^j, 1\leq j \leq |\agentVec|$ is the set of $n$-agent stage games,
$\pmb{A}=\times_{\agent\in\agentVec}\mathcal{A}^{\agent}$ is the set of joint actions,
$\mathcal{R}$ is the reward function that determines the payoff for all the agents $\agentVec$ as 
$\reward^{\agentVec}:
\mathcal{S}^1\times...\times\mathcal{S}^{|\agentVec|}\times\mathcal{A}^1\times...\times\mathcal{A}^{|\agentVec|}\rightarrow\mathbb{R}$, 
$\pmb{P}$ is a stochastic transition function over the state space $\pmb{S}$. An MDP is a 1-agent SG; an MDP thus has the simpler structure $<\mathcal{S}, \mathcal{A}, P, \mathcal{R}, \gamma>$.

In an environment with multiple intersections, the system contains the general environment $\environmentVec$ containing a set of four-leg intersections, each of which is represented as $\agent\in\agentVec$. For the general environment $\environmentVec$, at every time step $t$, the goal of the system control is to provide joint actions $\actionVec^*_t=(\action^1_t,...,\action^{|\agentVec|}_t)\in\pmb{A}$ that maximize the system reward $r^{\agentVec}_t$. 

\end{problem}

Figure~\ref{fig:system} illustrates the basic idea of reinforcement learning framework in traffic light control problem. The environment is the traffic conditions on the roads and agents control the traffic signals.  The goal of a traffic signal agent $\agent$ controlled with RL is to learn the optimal action value function $Q^*(s,a)$.  Each time state $t$, a description of the environment (e.g., signal phase, waiting time of cars, queue length of cars, and positions of cars) will be generated as the state $\staterep_t$. The agent will make prediction on the next action $\action_{t}$ to take: $\action_{t} = argmax_{\action \in \mathcal{A}}Q(a;\staterep_t)$, where the action could be changing to certain phase in single intersection scenario, and be joint action vector in multi-intersection scenario. The action $\action_t$ will be executed in the environment and a reward $\reward_{t}$ will be generated, where the reward could be defined on the level of individual intersections or a group of intersections within the environment.


\begin{figure}[t]
  \centering
   \includegraphics[width=0.85\textwidth]{fig/system.pdf}
   \vspace{-1mm}
     \caption{Reinforcement learning framework for traffic light control.}
     \vspace{-3mm}
    \label{fig:system}
\end{figure}

% \subsubsection{Categorization of reinforcement learning methods}

% \begin{itemize}
% \item Model-based vs. model-free. Most reinforcement learning systems are built upon Markov Decision Process. However, depending on their modeling philosophy, they can be divided into two categories: model-based and model-free~\cite{ADBB17, KLM96}. For a problem with large state and action space, it is usually difficult to conduct millions of experiments to cover all possible cases. Model-based methods try to model the transition probability among states explicitly and this can be used to sample the environment more efficiently (agent can acquire data samples according to this transition matrix). Concretely, given this model, you will know which state the each action will take the agent to. In contrast, model-free methods directly estimate the reward for state-action pairs, and choose the action based on this. Hence, model-free methods can be used even the transition probability is hard to model.

% \item Tabular methods vs. approximation methods. For small-scale discrete reinforcement learning problem in which the stat-action pairs can be enumerated, it is a common practice to use a table to record the value functions, policies or models. However, for large-scale or continuous problem (state or action is continuous), it is not realistic to enumerate all the state-action pairs. In this case, we need to estimate the value function, policy or model using an approximation function of the state and action.

% \item Value based vs. policy based vs. Actor-Critic. Depending on the different ways of estimating the potential reward and select action, reinforcement learning methods can be categorized into the following three categories: 

% \begin{itemize}
% \item Value based methods approximate the state-value function or state-action value function (i.e., how rewarding each state is or state-action pair is), and the policy is implicitly obtained from the learned state-action value function.
% \item Policy based methods directly update the policy (e.g., a vector of probabilities to conduct actions under specific state) parameters along the direction to maximize a predefined objective (e.g., average expected reward).
% \item Actor-Critic methods combine above-mentioned methods with an actor controls how our agent behaves (policy-based), and the critic measures how good the action taken is (value-based).
% \end{itemize}
% \end{itemize}

% \subsection{Reinforcement learning for traffic light control}


% \subsubsection{Problem definition}
% \begin{problem}[RL for Isolated-intersection Traffic Signal Control]
% \label{prob:RLI}
% For a single intersection, the goal of a traffic signal agent $\agent$ controlled with RL is to learn the optimal action value function $Q^*(s,a)$. At every time step $t$, $\agent$ observes from its environment $\environment$, takes action $\action_t$ that maximize the reward $r_t$ (i.e., the performance of the intersection), given the state $\staterep_t$ (describing the positions of vehicles near this intersection). %This paper consider a signalized four-leg intersection as $\environment$.
% \end{problem}

% \begin{problem}[RL for Multi-intersection Traffic Signal Control]
% \label{prob:RLM}
% In our problem, the system contains the general environment $\environmentVec$ containing a set of four-leg intersections, each of which is represented as $\agent\in\agentVec$. For the general environment $\environmentVec$, at every time step $t$, the goal of the system control is to provide joint actions $\actionVec^*_t=(\action^1_t,...,\action^{|\agentVec|}_t)\in\pmb{A}$ that maximize the system reward $r^{\agentVec}_t$. 
% \end{problem}

\nop{
\subsection{Challenges}
\begin{itemize}
\item Capture the situation on the road and convert it to values. State and reward definitions.
\item Selection of action scheme. Timed action, actuated action? 
\item Deal with continuous large state space. One way is to get discretize then use tabular methods, the other is to use continuous methods (approximation methods).
\item Deal with multiple intersections. Consider other intersections. Consider interactions between intersections.
\end{itemize}
}
\subsubsection{Challenges}
The main challenge of using RL for traffic signal control is how to formulate the problem under the framework of RL. Here are some key points:

\begin{itemize}
\item Reward design. As RL is learning to maximize a numerical reward, the choice of reward determines the direction of learning.   
\item State design. State captures the situation on the road and convert it to values, thus the choice of states should sufficiently describe the environment.
\item Selection of action scheme. Timed action, or actuated action? 
\item Coordination.  In urban environments, signals are often in close proximity and this complicates the signal timing problem. Specifically, vehicles departing from one signal influence the arrival pattern of vehicles to the next downstream intersection. Thus, optimizing of signal timings for adjacent traffic signals must be done jointly.
\end{itemize}

\subsection{State definitions}
One of the most important issues to be considered when designing a reinforcement learning based method is that of determining how the state of the environment will be represented to the agent. Various different approaches to defining the environment state in reinforcement learning for traffic signal control problems have been proposed in the literature, with each having its own relative merits.
\begin{itemize}
    \item Queue length: the total number of waiting vehicles. While there is different definitions on a "waiting" state of a vehicle. In~\cite{wei2018intellilight}, a vehicle with a speed of less than 0.1 m/s is considered as waiting; in ~\cite{BSSN+05,KWBV08}, a vehicle without movement in terms of position is considered as waiting.
    \item Waiting time. The waiting time is defined as the time a vehicle has been waiting. Variations on this definition is different in when to consider the waiting time: in~\cite{wei2018intellilight}, they consider the waiting time starting from the last time stamp the vehicle moved, while~\cite{Wier00} consider the waiting time from the time the vehicle enters the system.
    \item Delay. Delay is defined as the time a vehicle travels below a threshold speed, which varies in different maximum speed scenarios.
    \item Traffic flow rate. The traffic flow rate is defined as the number of vehicles entering the system within certain time periods.
    \item Elapsed time: elapsed time of the current phase.
    \item Position of vehicles. The positions of vehicles are usually integrated through a image representation or through the location of the vehicle nearest to the intersection.
    \item Phase: The phase information is usually integrated into the state through a index of current phase in the pre-defined signal phase groups\cite{EAA13,wei2018intellilight,VaOl16} or through a mask on the rest of the states, i.e., the queue length of each phase~\cite{MaDH16}.
\end{itemize}
\begin{table}[htbp]
\caption{State definitions}
\begin{center}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
State  & References \\
\midrule
Queue length & \cite{APG03, AMB11, AMB14,wei2018intellilight, XXL13,CBYT11, ElAb10, ElAb12, EAA13,BSSN+05,Saca10,SCGC08,BGS10,MaDH16} \\ \midrule
Waiting time & \cite{Wier00,PBTB+13,BPT14,wei2018intellilight} \\ \midrule
Volume & \cite{wei2018intellilight,PraB11}\\ \midrule
Delay &  \cite{ALUK10, BWKG10, IKKK06, KWBV08, SSPN+05, WVVK04, WVVK04-2}\\ \midrule
Traffic flow rate & \cite{BGS10}  \\  \midrule
Elapsed time & \cite{BPT14,PraB11,EAA13} \\ \midrule
Congestion & \cite{BSSN+05} \\ \midrule
Position of vehicles & \cite{KWBV08, BSSN+05, VaOl16,wei2018intellilight, XXL13} \\ \midrule

Phase  & \cite{EAA13,wei2018intellilight,VaOl16,MaDH16} \\ 
\bottomrule
\end{tabular}
\label{tab:state-definitions}
\end{center}
\end{table}

\subsection{Reward functions}
Choosing an appropriate reward function is equally important as the choice of state representation when designing an reinforcement learning agent. These issues are somewhat interrelated, in that the reward received by an agent is often related to the difference in utility between the current and previous states, i.e. the agent is rewarded for actions that improve the state of the environment. Equivalently, we can think of optimizing some parameter as the agent's objective, and this objective is specified in the reward function. As a common practice, the reward function is usually defined as a weighted sum of the factors in Table~\ref{tab:reward}. And all the studies only come up with ad-hoc weights on different factors.

\begin{itemize}
    \item Queue length: Minimizing the queue length is somehow equivilant to minimizing total travel time, and could prevent from the queue spillback.
    \item Waiting time. A typical reward function considers the negative value of the waiting time experienced by the vehicles between two time points. It could either be two successive decision time points or the time entering the system and the current decision time.
    \item Delay or Speed restriction. Delay is defined as the time a vehicle travels below a threshold speed, which varies in different maximum speed scenarios. While minimizing delay is equal to maximizing the average speed, it does not consider the waiting time of vehicles and may lead to situations where it is optimal to never open up a road as long as there are cars moving on the other road. Thus,.
    \item Number of stops. Reducing the cumulative delay or balancing queue lengths does not guarantee minimizing the total number of stops. A reward can be defined as the negative of the number of stops that occurred between two successive decision points.
    \item Other concerns. There should not be many emergency stops and the learned policy should not lead to flickering, i.e. changing light states on each time step, since these two things make for unpleasant and unsafe driving. Furthermore, jams or would-be collisions should be prevented.
\end{itemize}

\begin{table}[htbp]
\caption{Reward functions}
\label{tab:reward}
\begin{center}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
Reward  & References \\
\midrule
Queue length & \cite{MaDH16,VaOl16,BSSN+05,KWBV08,wei2018intellilight,PraB11,Saca10,SCGC08}\\ \midrule
Waiting time & \cite{AMB11, AMB14, MaDH16,VaOl16,Wier00, APG03}\\ \midrule
Delay & \cite{BPT14,ElAb10, ElAb12,VaOl16} \\ \midrule
Accident avoidance & \cite{VaOl16}\\ \midrule
Speed restriction  &  \cite{KhGo12,KhGE12}\\ \midrule
Number of stops & \cite{VaOl16}\\ \midrule
Throughput & \cite{Saca10,SCGC08}\\ 
\bottomrule
\end{tabular}
\label{tab:reward-functions}
\end{center}
\end{table}

\subsection{Action definitions}
Earlier RL methods learn to set phase times for next cycle given the current traffic conditions. However, since the cycle length is usually too long for the dynamic changing traffic, recent RL methods learn to decide the next phase. Now there are two other phasing sequence schemes as shown in Table~\ref{tab:action-definitions}: fixed phasing sequence, in which a fixed order of phases is followed, and variable phasing sequence, in which the phasing sequence is not predetermined. 

In a fixed phasing sequence,  the action is a binary number which indicates RL agents either decides the time for different phases in a cycle or decides whether change the current signal to the next phase. One of the strengths of fixed phasing sequence is that the reliability of a phase sequence is good for drivers in practice. 

In variable phasing sequence, the action is the phase index that should be taken next. the signal timing is more flexible and the agent is learning to select a phase to change to, without assumptions that the signal would change in a cycle.

\begin{table}[htbp]
\caption{Action definitions}
\begin{center}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
Action & References \\
\midrule
Set phase times & \cite{AMB11, AMB14,Saca10,SCGC08} \\ \midrule
Change to next phase & \cite{VaOl16,wei2018intellilight,PBTB+13,BPT14} \\ \midrule
Determine phase to change & \cite{BSSN+05,KWBV08,ALUK10} \\
\bottomrule
\end{tabular}
\label{tab:action-definitions}
\end{center}
\end{table}

\subsection{RL Approaches}

\subsubsection{Model-based vs. model-free.} 
Most reinforcement learning systems are built upon Markov Decision Process. However, depending on their modeling philosophy, they can be divided into two categories: model-based and model-free~\cite{ADBB17, KLM96}. For a problem with large state and action space, it is usually difficult to conduct millions of experiments to cover all possible cases. Model-based methods try to model the transition probability among states explicitly and this can be used to sample the environment more efficiently (agent can acquire data samples according to this transition matrix). Concretely, given this model, you will know which state the each action will take the agent to. In contrast, model-free methods directly estimate the reward for state-action pairs, and choose the action based on this. Hence, model-free methods can be used even the transition probability is hard to model.

In the context of traffic signal control problem, to develop a model-based model, it requires the full dynamics of the system to be known or modeled, including the position, speed, and acceleration of all vehicles, and the operations of all the traffic signals. For one thing, people's driving behavior can be really different and hard to predict. For another thing, these data themselves, are highly depended on a comprehensive sensor system which need to installed on every vehicle. Therefore, these massive data can be extremely hard to collect. To the best of our knowledge, most of the current literature select the model-free approach, without modeling the transitions between states.

\paragraph{Value based methods vs. policy based vs. Actor-Critic.}
Depending on the different ways of estimating the potential reward and select action, reinforcement learning methods can be categorized into the following three categories: 

\begin{itemize}
\item Value based methods approximate the state-value function or state-action value function (i.e., how rewarding each state is or state-action pair is), and the policy is implicitly obtained from the learned state-action value function.
\item Policy based methods directly update the policy (e.g., a vector of probabilities to conduct actions under specific state) parameters along the direction to maximize a predefined objective (e.g., average expected reward).
\item Actor-Critic methods combine above-mentioned methods with an actor controls how our agent behaves (policy-based), and the critic measures how good the action taken is (value-based).
\end{itemize}

Under the scenario of traffic signal control, the action can be defined as shown in Table~\ref{tab:action-definitions}. Hence, the learned policy represents the probabilities to take different actions under certain state. Value based methods, including Q-learning~\cite{AMB11, CBYT11}, and DQN~\cite{VaOl16, wei2018intellilight}, directly model the state-values or state action values (e.g., under the current traffic situation, how much average speed increase/decrease will take into effect if one action is conducted). In this way, the state and reward can be directly fed into the model without extra processing. However, these methods are usually combined with an $\epsilon$-greedy action selection methods, and hence will result in a nearly deterministic policy when $\epsilon$ finally decays to a small number (i.e., it is deterministic which action will be conducted under certain states). In addition, these methods can only deal with discrete actions, because it requires a separate modeling process for each action. In contrast, policy based methods, like policy gradient~\cite{mousavi2017traffic}, try to learn a probability distribution of different actions under certain state. The advantage of this is that, it does not require the action to be discrete. It can learn a stochastic policy and keep exploring potential more rewarding actions. However, because the probability represents a relative order of the reward, it requires the fed state-action-reward data to be processed carefully. Sometimes, these methods may lead the agent to a local optima~\cite{SMSM00}. Actor-Critic methods~\cite{PraB11, aslani2017adaptive, aslani2018developing}, which are designed to combine the aforementioned two groups of methods, utilize the strengths of both value function approximation and policy optimization, have shown good performance in traffic signal control problems. Note that, however, to the best of our knowledge, there is no systematic experimental comparison of these three groups of methods under the problem setting of traffic signal control.

\begin{table}[hbt]
\caption{Value-, policy- and actor-critic-based methods}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
                & References \\ \midrule
Value-based     & \cite{AMB11, CBYT11, VaOl16, wei2018intellilight}    \\
Policy Gradient & \cite{PraB11, mousavi2017traffic,Casa17}           \\
Actor-Critic    &  \cite{PraB11, aslani2017adaptive, aslani2018developing}       \\ 
\bottomrule
\end{tabular}
\end{table}

\paragraph{Tabular methods and approximation methods} 
For small-scale discrete reinforcement learning problem in which the stat-action pairs can be enumerated, it is a common practice to use a table to record the value functions, policies or models. However, for large-scale or continuous problem (state or action is continuous), it is not realistic to enumerate all the state-action pairs. In this case, we need to estimate the value function, policy or model using an approximation function of the state and action.


The choice of tabular methods and approximation methods mainly depends on whether the state feature space can be converted to meaningful discrete space. In the problem scenario of signal control,  earlier methods use some simple state features (which can be converted to discrete state values) and employ tabular Q-learning \cite{APG03,ElAb10} to learn the value function. These methods thus cannot scale up to a large state space for complicated scenarios in traffic signal control. In addition, tabular methods will treat samples with similar features as two completely different states, which will decrease the efficiency of utilizing samples in training. To solve these problems, recent studies propose to apply function approximation using continuous state representations\cite{BPT14,ADBB17,wei2018intellilight,MaDH16,VaOl16,AMB14,BaKl14,EAA13,ElAb12,KhGo12,ALUK10}. The function approximation could be achieved by multiple machine learning techniques, like tile coding or deep neural networks. These methods are able to utilize the samples with similar state values more efficiently and deal with more informative features with continuous ranges, e.g., position of vehicles.

\begin{table}[hbt]
\caption{Tabular methods and approximation methods}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
                                                                & References \\ \midrule
Tabular methods                                                 & \cite{Wier00,WVVK04,WVVK04-2,APG03,ElAb10}  \\  \midrule
Approximation methods & \cite{BPT14,ADBB17,wei2018intellilight,MaDH16,VaOl16,AMB14,BaKl14,EAA13, ElAb12,KhGo12,ALUK10}  \\ \bottomrule
\end{tabular}
\end{table}



\subsubsection{Coordinated Strategies}
Coordination could benefit the signal control for multi-intersection scenarios. Since recent advances in RL improve the performance on isolated traffic signal control~\cite{VaOl16,wei2018intellilight}, efforts have been performed to design strategies that cooperate multiple RL agents. 

\begin{itemize} 

\item Single agent. A straightforward solution is to use one agent to control all the intersections~\cite{PraB11}. 

\item Implicit coordination through individual RL. There are also a line of studies that use individual RL agents to control the traffic signals in the multi-intersection system~\cite{ElAb12,ALUK10,DrSt06,SBPB+06,EAA13,DrSt06,Wier00}. Instead of explicitly design a module for coordination, these methods cooperates implicitly by sensing part of the environment and adapt (or react) to it accordingly and eventually form several subgroups of synchronization. These approaches use neither explicit communication nor a manager agent to resolve conflicts. These methods are more scalable, since each agent makes its own decision based on the information from itself and neighboring intersections without explicit coordination. However, when multiple agents are interacting with the environment at the same time, the non-stationary impacts from neighboring agents will be brought into the environment and the learning process usually cannot converge to stationary policies if there are no communication or coordination mechanisms among agents~\cite{Bish06,NoVr12}.  In highly dynamic environments, an agent might not have the time to perceive a change and adapt to it before the environment has already changed again. In reasonably well behaved scenarios, the adaptive approach with formation of several mini green waves has performed well compared to arterial-based, fixed green waves. 

\item Coordination through communication. Instead of heuristically adding neighboring states into the target agent, \cite{GCN18} proposes to use Graph Convolutional Network to incorporate communications through learning neighbors' hidden state for the target agent. This method could also learning multi-hop influences between intersections.

\item Joint action modeling through coordination graph. \cite{KWBV08} and \cite{VaOl16} consider explicit coordination mechanisms between learning agents using coordination graphs, extending \cite{Wier00} using max-plus algorithm. A coordination graph~\cite{GLP02}, which can be used to describe the dependencies between agents, is an undirected graph $G = (V, E)$ in which each node $i \in V$ represents an agent and each edge $e(i, j) \in E$ between agents i and j indicates a dependency between them. Max-plus algorithm then approximates the optimal joint action by iteratively sending locally optimized messages between connected nodes in the graph. While in state $s$, a message from agent $i$ to neighboring agent $j$ describes a local reward function for agent $j$ and is defined by:
$u_{ij}(a_j)=max_{a_i}\{ Q_{ij}(s,a_i,a_j)+\Sigma_{k\in \Gamma(i)\\j} u_{ki}(a_i)\}$, where $\Gamma(i)\\j$ denotes all neighbors of $i$ except for $j$. The message approximates the maximum value agent $i$ can achieve for each action of agent $j$ based on the function defined between them and incoming messages to agent $i$ from other connected agents (except $j$). Once the algorithm converges, each agent $i$ can select the action $a^*=argmax_{a_i}\Sigma_{j\in\Gamma(i)}u_{ji}(a_i)$. This method need to pre-define the $Q_{ij}(s,a_i,a_j)$

% \item Multi-level agent. \cite{YCTS05} and~\cite{FrGh03} propose to use hierarchical multi-agent RL for global optimization on traffic signal control.  A hierarchical multiagent system with three levels is proposed in~\cite{FrGh03}. In the first level, local traffic agents represent intersections; these are responsible for providing appropriate traffic signal timing which allows traffic to pass based only on local traffic patterns. Because the local optimum may not be a good one when observed from another perspective, there is a second level in the system, in which a coordinator traffic agent supervises a few local traffic agents. According to the authors, a coordinator traffic agent should provide a means by which the optimal local signal pattern can be slightly modified to accommodate the global performance.However, in the paper, it is not discussed how this can be achieved. The authors mentioned that once a local agent calculates its local optimum, the corresponding central agent is informed and adjusts local solutions to meet concerns at the central level. However, details are not given.
\end{itemize}

\begin{table}[hbt]
\caption{Different coordination methods for traffic signal control}
\begin{tabular}{p{3cm} p{12cm}}
\toprule
                       & References \\ \midrule
Single Agent           & \cite{PraB11}  \\ \midrule
Individual RL          &  \cite{ElAb12,ALUK10,SBPB+06,EAA13,DrSt06,Wier00,WVVK04-2} \\ \midrule
Communication          & \cite{GCN18}            \\ \midrule
Joint Action Modeling  & \cite{KWBV08, VaOl16}   \\    \bottomrule
\end{tabular}
\end{table}

 Explicitly coordinating through information sharing or multi-level agent offers many drawbacks. Current coordinated control requires prior knowledge of traffic patterns and road length to calculate optimal offsets, road structure information to build coordinated graph, etc. The obtained solutions are specific to the road network structure. When these features change (e.g., when new intersections are considered), the prevailing coordination policy must be created again. Centralized approaches can alleviate this but these result in large-scale optimization problems that are often not computationally feasible, especially in real-time. Information sharing approaches also rely on large communications networks to share information between signals, and such information is not feasible to obtain. 

\subsection{Learning efficiency techniques}
The key principle of RL is trial-and-error, which leads to longer learning time and more expensive computational resources. However, in real-world applications, such as traffic signal control, these costs may cause significant consequence (e.g., traffic congestion). Besides some general techniques that are proved to improve the learning efficiency for general RL applications (e.g., priority sampling, double DQN, etc.), several strategies are proposed to make the RL learn efficiently especially for traffic signal control problem.

\begin{itemize}
    \item Phase gate~\cite{wei2018intellilight}.
    \item Memory palace~\cite{wei2018intellilight}.
    \item Transfer agents~\cite{VaOl16}.
\end{itemize}


\subsection{Experiment setting}
In this section, we will introduce some aspects that will influence the performance of traffic signal control strategies: simulation environment, road network setting and traffic flow setting.
\begin{itemize}
    \item Simulation environment. Deploying and testing traffic signal control strategies involves high cost and intensive labor. Hence, simulation is a useful alternative prior to actual implementation. Simulations of traffic signal control often involve large and heterogeneous scenarios, which should account for some specific mobility models in a vehicular environment, including car following, lane changing and routing. Since mobility models can significantly affect simulation results, it is important that the simulated model is as close to reality as possible.
    \item Road network.
    \item Traffic flow.
\end{itemize}

\subsubsection{Simulation environment}
Various publicly available traffic simulators that are currently in use by the research community. In this section, we briefly introduce some open-source tools that are used in the current traffic signal control literature. Specifically, since RL-based methods requires more detailed state representation, most literature rely on microscopic simulation, in which movements of individual vehicles are represented through microscopic properties such as the position and velocity of each vehicle. Other proprietary simulators like Paramics, VISSIM and QualNet will not be introduced here. For a detailed comparison of the open-source simulators, please refer to~\cite{simulator11}.


\begin{itemize}
    \item The Green Light District (GLD)~\footnote{https://sourceforge.net/projects/stoplicht/}. GLD is an open-source traffic flow simulator which can be used to evaluate the performance of AI traffic light controller algorithms and co-learning navigation algorithms for cars. Vehicles enter the network at edge nodes and each edge node has a certain probability of generating a vehicle at each timestep (spawn rate). Each generated vehicle is assigned one of the other edge nodes as a destination. The distribution of destinations for each edge node can be adjusted. There can be several types of vehicles, defined by their speed, length, and number of passengers.
    \item The Autonomous Intersection Management (AIM)~\footnote{http://www.cs.utexas.edu/~aim/}. AIM is a microscopic traffic simulator which mainly supports a Manhattan topology of North-South and East-West multi-lane roads joined by a number of intersections. Developed by the Learning Agents Research Group at the University of Texas at Austin, AIM supports vehicles navigate an intersection, accelerate, and decelerate, as well as subtle details including variable vehicle sizes.
    \item Simulation of Urban MObility (SUMO)~\footnote{http://sumo.sourceforge.net}. SUMO is an open-source program for traffic simulation, mainly developed by Institute of Transportation Systems, located at German Aerospace Center. Among other features, it allows the existence of different types of vehicles, roads with several lanes, traffic lights, graphical interface to view the network and the entities that are being simulated, and interoperability with other applications at run-time through an API called TraCI. Moreover, the tool is considered to be fast, still allowing a version without a graphical interface where the simulation is accelerated putting aside visual concerns and overheads. Also, it allows importing real-world raod networks from OpenStreetMap and does not require the vehicles enters the system from the edge nodes.
\end{itemize}

\begin{table}[hbt]
\caption{Different simulators used in literature for RL-based traffic signal control }
\label{tab:simulators}
\begin{tabular}{llll}
\toprule
    & Latest update & Developed by & References \\ \midrule
GLD &   1.0 (Jan. 2005)   & \begin{tabular}[c]{@{}l@{}} University of Groningen,\\ The Netherlands \end{tabular}  &  \begin{tabular}[c]{@{}l@{}} 
\cite{Wier00,WVVK04,WVVK04-2}\\
\cite{ BSSN+05, SSPN+05}\\
\cite{KWBV08,IKKK06} \\
\cite{BWKG10, PraB11}
\end{tabular}     \\ \midrule
SUMO &  1.1.0 (Dec. 2018) &   \begin{tabular}[c]{@{}l@{}}  German Aerospace Center (DLR) \\
Institute of Transportation Systems\end{tabular}            & 
\begin{tabular}[c]{@{}l@{}} 
\cite{VaOl16,wei2018intellilight}  \\ 
\cite{mousavi2017traffic, MaDH16} \\
\cite{GCN18}
\end{tabular}     \\ \midrule
AIM  &  1.0.4 (Mar. 2017)   & \begin{tabular}[c]{@{}l@{}} University of Texas at Austin,\\ USA\end{tabular} & 
\begin{tabular}[c]{@{}l@{}}
\cite{aslani2017adaptive, aslani2018developing} \\
\cite{PBTB+13, BPT14} 
\end{tabular} \\ \midrule
Others & \multicolumn{3}{l}{ \begin{tabular}[c]{@{}l@{}} Matlab~\cite{ALUK10}, Paramics~\cite{EAA13,ElAb12} \\
Aimsun~\cite{AMB11,Casa17}  \end{tabular} } \\
\bottomrule
\end{tabular}
\end{table}


\subsubsection{Road network}


\begin{table}[htb]
\caption{Size of road network in literature for RL-based traffic signal control }
\label{tab:exp-network}
\begin{tabular}{lll}
\toprule
                   & Intersections   & References \\ \midrule
Synthetic network & $<10$     & \begin{tabular}[c]{@{}l@{}} \cite{Wier00,VaOl16,MaDH16}\\
                                                            \cite{ALUK10,DrSt06,GCN18} \end{tabular}        \\ \cmidrule{2-3}
                   & $10-20$   & \cite{WVVK04,WVVK04-2,KWBV08,BSSN+05,BWKG10}           \\ \cmidrule{2-3}
                   & $>=20$    &  
                   \begin{tabular}[c]{@{}l@{}}
                    \cite{AMB11,aslani2018developing}(50)  \\ 
                    \cite{aslani2017adaptive,PBTB+13, BPT14} (50) 
                \end{tabular}
                \\ \midrule
Real road network  & \multicolumn{2}{l}{
                            \begin{tabular}[c]{@{}l@{}}
                        \cite{ElAb12,EAA13}(59) \\
                        \cite{SCGC08}(64),~\cite{Casa17}(43)
                        \end{tabular} 
                        }
                        \\ 
                   \bottomrule        
\end{tabular}
\end{table}

\subsubsection{Traffic flow}

\begin{table}[htb]
\caption{Traffic flow used in literature for RL-based traffic signal control. The traffic with arrival rate less than 500 vehicles/hour/lane is considered as light traffic in this survey, otherwise considered as heavy.}
\label{tab:exp-traffic}
\begin{tabular}{lccl}
\toprule
                &                &          & References \\ \midrule
Synthetic data  & light          & fixed         &  \begin{tabular}[c]{@{}l@{}}
                                                        \cite{KWBV08,PraB11,AMB11}        \\ 
                                                        \cite{VaOl16,MaDH16, GCN18} 
                                                    \end{tabular} \\ \cmidrule{3-4}
                &                & dynamic       &  \cite{MaDH16}         \\ \cmidrule{2-4}
                & heavy          & fixed         &  \begin{tabular}[c]{@{}l@{}}
                                                        \cite{SSPN+05, AMB11}          \\
                                                        \cite{Wier00,WVVK04,WVVK04-2}
                                                    \end{tabular} \\ \cmidrule{3-4}
                &                & dynamic       &    \cite{BWKG10}        \\ \midrule
Real-world data & \multicolumn{3}{c}{\cite{ElAb12,EAA13,Casa17,wei2018intellilight}} \\
\bottomrule
\end{tabular}
\end{table}


\subsection{RL for traffic signal control is still challenging}

In summary, current RL-based methods have the following drawbacks. (1) They mainly focused on using different complex reward or state definitions to improve the empirical performance, without connection with classic transportation theory or methods. (2) Current coordination only considers regional control up to 60 intersections, while city-wide control requires a scalable control method for thousands of traffic signals. (3) Current methods only test on simulated scenarios in under-saturated traffic and lack systematic test under different traffic conditions. (4) Current RL-based methods usually do not consider learning efficiency, which is of great importance when applying RL in the physical world.

\paragraph{Formulation of RL agent}
A key question for RL is how to define reward and state. In existing studies~\cite{Wier00,VaOl16,wei2018intellilight}, a typical reward definition for traffic signal control is a weighted linear combination of several components such as queue length, waiting time, number of switches in traffic signal, and sum of delay. The state include components such as queue length, number of cars, waiting time, and current traffic signal. In recent work~\cite{VaOl16,wei2018intellilight}, images of vehicles' positions on the roads are also considered in the state.  

However, all of the existing work take an ad-hoc approach to define reward and state. Such an ad-hoc approach will cause several problems that hinder the application of RL in the real world. First, the engineering details in formulating the reward and state could significantly affect the results. For example, if the reward is defined as a weighted linear combination of several terms, the weights on each terms are tricky to set and the minor difference in weight setting could lead to dramatically different results. Second, the state representation could be in a high-dimensional space, especially when using traffic images as part of the state representation~\cite{VaOl16,wei2018intellilight}. Such a high-dimensional state representation will need much more training data samples to learn and may not even converge. Third, there is no connection between existing RL approaches and transportation methods. Without the support of transportation theory, it is highly risky to apply these purely data-driven RL-based approaches in the real physical world. 

\paragraph{Learning cost}

While learning from trial-and-error is the key idea in RL, the learning cost is RL is fatal for real-world applications. Although RL algorithms are very useful to learning good solutions when the model of environment is unknown in advance~\cite{RiAn98,watkins1989learning}, the solutions may only be achieved after an extensive numbers of trials and errors, which is usually very time consuming. Existing RL methods for games (e.g, Go or Atari games) yield impressive results in simulated environments, the cost of error in traffic signal control is critical, even fatal in the real world. Therefore, how to learn efficiently (e.g., learning from limited data samples, sample training data in an adaptive way, transfer learned knowledge) is a critial question for the application of RL in traffic signal control.

\paragraph{Delayed reward}
 Delayed reward has been one of the most widely discussed question in reinforcement learning. This phenomenon exists in the Go game and many Atari games. Unlike in these games, where people sometimes assign the final score of an episode to all the actions associated with this episode, the action in the traffic signal control problem may have a affecting time interval that need to be discovered. This affecting time interval brings two problems: (1) one action may still have effect after several steps of actions; (2) the reward at each timestamp is a result of the combination of several consequent actions. What's more, this affecting time interval may change due to different external factors, e.g., weather. Under this assumption, unlike Go, if we simply run an episode and assign the final reward to each associated action, this reward will be very noisy, and it will require too many data samples, given the large state space of this problem. Therefore, it is essential to come up of a great way of assigning the delayed reward.

\nop{
\paragraph{Lifelong learning to adapt to change}
}
 
\subsection{Summary}



==> bk_transportation.tex <==
% basicTLCS.tex
\section{Methods in transportation engineering}
\label{sec:transportation}

In this section, we introduce the methods in transportation engineering from three categories:  (1) pre-timed control which pre-defines the signal plans offline; (2) actuated control adjusts traffic signals according to the rules and real-time traffic data; and (3) adaptive control dynamically choose the traffic signal plan. 


    %Isolated vs. coordinated control. Modern urban traffic-control system is not only just signal plan of intersections, but also signal coordination of a large traffic networks, which includes arterial and grid-like regions. Coordination is largely a strategic approach to synchronize signals together to meet specific objectives. While there are numerous objectives for the coordination of traffic signals, common objectives are stated succinctly in ~\cite{koonce2008traffic}: The intent of coordinating traffic signals is to provide smooth flow of traffic along streets and highways in order to reduce travel times, stops and delay, which reduces fuel consumption and improves air quality. Various performance measures can be used to evaluate signal coordination. Isolated intersection performance measures include delay, queue length, and safety; however, performance measures for coordinated systems may be slightly different. Evaluation methods include the number of stops reduced for the main street through movements or queue management. With the modern signal controller, coordination is accomplished by adding a layer of logic (that is, coordination logic compliments some basic features such as when a phase can begin or end) to the basic actuated logic used for isolated signal timing operations. In previous sections, the details of the controller settings were limited to those applied at isolated or independent intersections (cycle length, green split, maximum green, pedestrian timing, etc).

\textcolor{red}{jessie:pre-timed control does not need to compute offline}


\subsection{Pre-timed Control}
Pre-timed control methods compute the signal cycle, including its time duration and order of phases offline using historical traffic volumes, and then deployed online. 

\subsubsection{Isolated intersection control}
Isolated intersection control considers the signal control on one single intersection. This may be appropriate for signalized intersections that are isolated and not part of a larger control network (e.g. junctions in small towns)
One of the widely used method is from~\cite{koonce2008traffic} to minimize the total delay or maximize the intersection capacity. To determine a signal timing plan for pre-timed control in traffic engineering, there are the following essential elements:
\begin{enumerate}
\item Select an effective phase plan and sequence 
\begin{itemize}
\item  Determine how left turns should be treated and select proposed phasing plan. Usually a left-turn phasing is added when the left-turn flow is above a manually designed threshold.
\end{itemize}
\item Determine vehicular signal needs 
\begin{itemize}
\item Determine yellow and all-red times. This allows vehicles to stop safely or pass the intersection before conflicting vehicles are given green light.
\item Convert all volumes to through vehicle equivalents. This provides common basis since saturation flows are usually unknown at this stage.
\item Determine critical volume. Based on through vehicle equivalents per lane for all movements, it check all paths for largest sum of volumes.
\item Determine lost times. This is usually determined by expert knowledge.
\item Determine cycle length. The selection of a cycle length affects intersection capacity and delays. Longer cycle lengths can increase capacity, but only marginally. Shorter cycle lengths usually result in reduced delays. Thus, the objective of choosing a cycle length is to determine the smallest value of cycle length that provides the desired level of vehicular capacity at the intersection while being appropriate for the needs of other users such as pedestrians. 

Much of early research regarding cycle length selection recommended evaluating the intersections identifying the critical intersection which was typically the intersections with the highest demand. A desired cycle length is calculated based on the lost time, saturation flow, and traffic demand at the intersections, which optimize the total travel time of vehicles. The traditional models use Webster's model to determine optimal cycle length as Equation~\ref{eq:pre-timed}.
\nop{
\begin{equation}
\label{eq:pre-timed-webster}
    C_{des} = \frac{1.5L+5}{1.0-Y}
\end{equation}
where  $C_{des}$ is desirable cycle length (sec), $L$ is total lost time per cycle (sec/cycle), and $Y$ is the critical lane volume divided bu the saturation flow, summed over the phases. There are other variants in deciding the optimum cycle length, refering to XXX.
}

\begin{equation}
\label{eq:pre-timed}
    C_{des} = \frac{L}{1-\frac{V_c}{\frac{3600}{h} \times PHF \times (v/c)}}
\end{equation}

Here, $C_{des}$ is desirable cycle length (sec), $L$ is total lost time per cycle (sec/cycle), $PHF$ is the peak-hour factor which indicates ratio of volumes at peak hour over the average volumes. This could deal with the possible over-saturated situations in peak hour. $v/c$ is the target volume-to-capacity ratio for critical movements ranging from 0.85 to 0.95. $h$ is the saturation headway (sec/vehicle). $V_c$ is the maximum critical lane volume for intersection to accommodate in one hour (vehicle per hour per lane).

\item Determine green times. This is controlled by critical lane volumes and total lost time. The phase split percentage is equivalent with the percentage between critical lane volumes for a designated phase and the sum of critical lane volumes over all phases.
\end{itemize}
\item Determine pedestrian signal needs. This ensures the pedestrian can pass through the intersection.
\end{enumerate}

This kind of control strategies has some hidden assumptions:
\begin{itemize}
    \item the demand $d_j$ in lane $j$ should not be higher than the maximum possible flow assigned to this stream. Only then, the denominator in Equation~\ref{eq:pre-timed} is positive. 
    \item the steps above are sequentially computed, indicating the later steps are dependent of former steps, while this may not hold since they are mutually influenced.
    \item the parameters used for calculation should be pre-computed or known, while most of them are changing over time.
\end{itemize}

Instead of deciding a signal plan in a step-by-step way, ~\cite{improta1984control} consider the compatibility relations of involved streams as pre-specified and deliver the optimal staging, splits, and cycle time, so as to minimize total delay or maximize the intersection capacity. The resulting optimization problem is of the binary-mixed-integer-linear-programming type, which calls for branch-and-bound methods for an exact solution. 

\subsubsection{Coordinated multi-intersection control}
In order to optimize the early pre-timed signal control, some offline software were developed to calculate optimal signal settings for a single intersection or a network. The most popular representatives of this class of strategies for urban networks are outlined below.

\paragraph{MAXBAND} MAXBAND efficiently finds offsets for maximal bandwidth given cycle time, red times, signal distances, and street speed. The total bandwidth attained can be allocated between directions on the basis of flow. A basic symmetric, uniform-width bandwidth MAXBAND approach goes through the following steps:
\begin{enumerate}
\item Calculate cycle length $C_i$, phase split ($r_i$ is the ratio of red time over $C_i$, $g_i$ the ratio of green time over $C_i$, usually $g_i = 1 - r_i$) for each intersection $i$.
\item Determine the constraints. 
    \begin{itemize}
        \item Determine the constraints on cycle length. A widely-used practice is to let all the intersections have the same cycle length which equals to the maximum value of all cycle lengths of intersections, i.e. $C = max (C_1,C_2 \dots)$.
        \item Determine the constraints on the bandwidth of individual intersection. For simplicity, all the time intervals in the following refers to the ratio of time over the cycle length $C$.
        \begin{itemize}
        \item For each direction, the green time should be greater than the bandwidth. We have:
            \begin{subequations}
            \label{eq:MB-1}
            \begin{align}
                 w_i+b\leq 1-r_i,\ w_i>0 \\
                 \bar{w}_i+b\leq 1-\bar{r}_i,\ \bar{w}_i>0
            \end{align}
            \end{subequations}
            Here, $w_i (\bar{w}_i)$ is a variable of time interval between the end of red time of start of bandwidth on inbound (outbound) direction, $b$ is the bandwidth variable, and $r_i (\bar{r}_i)$ is the red time inbound (outbound) direction.
        \item For two different directions (inbound and outbound), usually the bandwidths for inbound and outbound are set equal.
        \end{itemize}
        \item Determine the temporal and spatial constraints on the relation between offsets of nearby intersections. 
            \begin{itemize}
                \item Temporal constraints. 
                    \begin{equation}
                    \label{eq:MB-2}
                        \phi(i,j) +\bar{\phi(i,j)} + \Delta_i - \Delta_j = m(i,j)
                    \end{equation}
                    Here, $\phi\ (\bar{\phi})$ is the inbound (outbound) offset between intersections, $\Delta$ is the intra-intersection offset between the inbound and outbound red time, $m(i,j)$ is an integer variable of the multiple over cycle length.
                \item Spatial constraints. The travel time a vehicle starting from one intersection to the other satisfy a function of the offset between them, the queue clearance time at the destined intersection and their red time.
                    \begin{subequations}
                    \label{eq:MB-3}
                    \begin{align}
                        \phi(i,j)+0.5*r_j+w_j+\tau_j = 0.5*r_i + w_i+t(i,j) \\
                         \bar{\phi}(i,j)+0.5*\bar{r}_j+\bar{w}_j = 0.5*\bar{r}_i + \bar{w}_i-\bar{\tau}_i+\bar{t}(i,j)
                    \end{align}
                    \end{subequations}
                Here, the $t\ (\bar{t})$ is the travel time inbound (outbound) between intersections, which is relevant to the street geometry and traffic speed.$\tau\ (\bar{\tau})$ is the queue clearance time at an intersection, which is relevant to the turn-in and generated traffic.
                \end{itemize}
    \end{itemize}
\item Solve the problem through integer linear programming techniques, i.e., find the optimal $b$, $w_i$, $\bar{w}_i$, $m_i$ that maximize:

    \begin{equation}
    b = \bar{b}
    \end{equation}
    
    subject to:
    
    \begin{equation}
        \begin{split}
        &Equation~\ref{eq:MB-1}, \ref{eq:MB-2}, \ref{eq:MB-3} \\
        &m_i = integer\\
        &b,\ \bar{b},\ w_i,\ \bar{w}_i \geq 0, i=,\dots,n
        \end{split}
    \end{equation}
\end{enumerate}

MAXBAND has been applied to several road networks in North America and beyond. A number of significant extensions have been introduced in the original method in order to consider a variety of new aspects. ~\cite{gartner1991multi} extends the basic problem to include asymmetric bandwidths in opposing direction, variable left-turn phase sequence, as well as decisions on cycle time length and link specific progression speeds. ~\cite{stamatiadis1996multiband} presents the new multi-band, multi-weight approach, which also incorporates all previous decision capabilities. 

\begin{itemize}
    \item Pros. MAXBAND uses relatively little inputs. The basic requirements are street geometry, traffic speeds, and green splits.  % Progression systems are operationally robust.
    Furthermore, various studies~\cite{wagner1969improved} and much practical experience~\cite{koonce2008traffic} have shown that bandwidth systems give good results in the field.
    \item Cons. As an offline method, this method requires a clear profile about the traffic flow in each intersection. This method may not be able to find a optimal solution or the optimal bandwidth could be very small that the coordination makes no difference. Only optimize the travel time mainly for traffic along corridors, neglecting the side roads. A person must invest substantial effort in learning how to formulate and solve problems in this way. 
\end{itemize}

\paragraph{TRANSYT}
TRANSYT was first developed by Robertson~\cite{robertson1969tansyt} but was substantially extended and enhanced later.
Initial signal settings of TRANSYT includes the pre-defined phase cycle, the minimum green duration for each phase of each intersection, and the initial choice of splits, offsets, and cycle time. 

The method proceeds in an iterative way: for given values of the decision variables (control inputs), i.e., of splits, offsets, and cycle time, the dynamic network model calculates the corresponding performance index based on a performance index that can be pre-defined or user-defined. A heuristic ``hill-climb'' optimization algorithm introduces small changes to the decision variables and orders a new model run, and so forth, until a (local) minimum is found.

TRANSYT allows the user to define the performance index used for optimization, including network delay, stops, fuel consumption and progression opportunities. During its optimization process, TRANSYT generates second-by-second flow profiles of vehicles on all links in the network, estimates queue lengths based on the profiles and analyzes these profiles to determine performance measures. This model considers the formation and dissipation of queues in space. In addition, it accounts for flow interactions on adjacent links through a step-by-step analysis of all links in the system. 

\paragraph{Others}
There are a number of computer programs that can be used to assist in selection of a cycle length. The Federal Highway Administration's Traffic Analysis Toolbox describes additional resources:~\cite{alexiadis2004traffic}.

\begin{itemize}
    \item PASSER program uses the concepts described in Webster's equation to determine the appropriate cycle length. The program uses a hill climbing algorithm to estimate delay at each intersection with the cycle length input to further quantify the performance of the system and maximize bandwidth using the pre-calculated splits as input to that model. At the optimization stage, it can find the cycle length, offsets, and phase sequences that produce maximum two-way progression. Essentially, PASSER uses the concepts described in Webster's equation for selection of cycle length and, "after calculating the minimum delay cycle length for all intersections in the arterial street, the largest minimum delay cycle length is selected as the shortest cycle length for the system and that the longest allowable cycle length should be no more than 10 to 15 seconds longer than the shortest allowable cycle length to minimize the excess delay at the non-critical intersections."~\cite{fambro1993implementation}.
    \item Synchro uses its algorithm to estimate arrivals at each intersection in the network and to calculate percentile signal delay, stops, and a queue penalty, which addresses the impact of queuing on arterial performance~\cite{husch2004trafficware}. The performance index is calculated for each cycle length based on the splits and offsets assumed within the model as constrained by the user. There are various steps to developing an ``optimal'' timing plan, but one of the limitations of this model is the inability to define the parameters within the Performance Index calculation.
\end{itemize}

\subsubsection{Summary of pre-timed control}
\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item Computationally efficient.
        \item Effective in networks with well-behaved traffic patterns, i.e., the traffic patterns are very similar over different time periods.
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item The signal plans are computed for a static situation, based on historical data. It is known that nowadays demand may not be constant, neither between days, nor during the day, nor in a given traffic direction. The operation of networks close to the saturation flow increases the chances of accidents which, in turn, contribute to unexpected patterns.
        \item Even if the computation itself is not manual, this is a complex task that requires a lot of expert knowledge as well as historical data. 
        \item Unsuitable for dynamic or unexpected traffic conditions. 
    \end{itemize}
     
\end{itemize}

\subsection{Actuated control}
\textcolor{red}{jessie: where is SOTL method?}
In general, pre-timed signals are the rule in urban areas for reasons of regularity, network organization, predictability, and reducing unnecessary delay. In areas with light traffic, actuated signals (push buttons, loop detectors) may be appropriate.

Actuated system controls the signal through detecting moving vehicles. When the time gap between detector activations (the detector is activated whenever a vehicle passes) exceeds exceeds some pre-defined threshold, current phase terminates~\cite{RPM04}. % The actuated signal timing is completely influenced by traffic volumes, and it is detected through sensors at all the approaches. It is mainly used at the intersections of the two main arterial streets.
% Generally traffic signals are operated in either actuated traffic mode or pre-timed mode or a combination of both. Pre-timed mode has series of intervals fixed with a particular duration and it will constantly repeat a preset cycle based on the timings. Actuated signals are operated at frequent intervals and it continuously detects the vehicular traffic volume.

There are two basic types of actuated signal control as follows:
\begin{itemize}
    \item \textit{Semi-actuated control} uses detection only for the minor traffic at an intersection, which is used under relatively uniform traffic flow. Semi-actuated control prioritizes the through movement of a major road and is not recommended on streets with frequent cross traffic or pedestrian demand from the minor approach unless a low cycle length is used.
    \item \textit{Fully-actuated control} refers to intersections for which all phases are actuated and hence, it requires detection for all traffic movements. which is used at the intersection where the traffic distribution keeps on changing. Fully-actuated signal control may be used where vehicle and pedestrian volumes vary considerably throughout the day. Fully-actuation can reduce the amount of delay by being responsive to ongoing shifts and patterns in the traffic system.
\end{itemize}

\subsubsection{Summary of actuated control}
\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item Computationally efficient.
        \item Effective in networks with well-behaved traffic patterns 
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item The signal changing rules are manual, which is a complex task that requires a lot of expert knowledge as well as historical data. 
        \item Unsuitable for dynamic or unexpected traffic conditions. 
    \end{itemize}
     
\end{itemize}

\subsection{Adaptive control}
The real-world traffic is dynamically changing, which hinders the applications of both pre-timed and actuated control. Adaptive control methods adjust signal timings in real time based on the current traffic conditions, demand, and system capacity. These methods require extensive surveillance (in the form of pavement loop detectors or surveillance cameras), and infrastructure that allows for communication with the central and/or local controllers. Currently nearly all adaptive systems are applied to coordinate multiple intersections. There are mainly two kinds of adaptive control methods, selection-based methods and optimization based methods. 

\subsubsection{Selection-based methods} Selection-based methods mainly take the real-time traffic condition, and select the next signal plan based on pre-defined signal plans. SCATS and SCOOT are the most-widely used methods in this category, where they take utilize performance models which map the traffic condition to the performance of the signal plan, and iteratively search all possible plans and select the one with the maximum performance index predicted by the predefined performance model. And Max-pressure is state-of-the-art method, which relies on the calculation of ``pressure'' for each pre-defined phase and directly choose to set green light for the phase with maximum pressure.

\paragraph{SCATS}
SCATS~\cite{lowrie1990scats} (Sydney Coordinated Adaptive Traffic System) consists of central computer, regional computer and local controllers. The local controller are grouped into subsystems, and each subsystem comprises one to ten intersections, operating on a common cycle length. The local controller utilizes detectors to gather the traffic movement information (i.e., traffic volume, time intervals of passing vehicles) from previous cycle optimize the traffic signal through adjusting the cycle length, phase split and offsets between adjacent intersections. It selects the signal plans which optimize its self-defined measurements like degree of saturation ($DS$) and traffic volume ($V$), detailed as follows:


\begin{subequations}
\begin{equation}
\label{eq:scats-ds}
    DS = \frac{t_{EG}}{t_G}=\frac{t_G-(t-t_0\times n)}{t_G}
\end{equation}
\begin{equation}
\label{eq:scats-v}
    V = \frac{DS\times t_G \times q_s}{3600}
\end{equation}
\end{subequations}
where $t_G$ is the green light time (in seconds), $t_{EG}$ is the effective green time during which there are vehicles passing through the intersection, $t$ is the detected time gap (the time interval vehicles pass the same detector), $t_0$ is the saturation time gap, which is a constant from 24-hour historical data, $n$ is the detected number of vehicles, $q_s$ is the saturation flow rate (vehicles per hour).

The measurements defined by SCATS have several strengths: 1) $DS$ is defined as $\frac{t_{EG}}{t_G}$, which is independent of the vehicle characteristics (e.g., vehicle length or vehicle speed). 2) $V$ is a surrogate of the number of vehicles passing through the intersection during the green time, which is also independent of the vehicles characteristics.


Specifically, the green split (i.e., the phase time ratio of all phases) of SCATS are based on several pre-defined signal plans which are usually set by domain experts or based on historical data. The selection of signal plans can be seen in Algorithm~\ref{alg:SCATS}.  If a signal plan is selected twice in 3 consecutive cycle, the signal plan will be used in the next cycle. The cycle length and offsets are also selected from several pre-defined plans.


\begin{algorithm}
\label{alg:SCATS}
\caption{Selection of Green Split}
\KwIn{Candidate signal plan set $A=\{a_j| j=1,\dots,N\}$ and current plan $a_c$}%, signal plan counter $C=[c_1,\dots,c_N]$}
\KwOut{Signal plan for next cycle}
% (Initialize signal plan counter)\\
% \For {$j=1;j \le N$}
% {
% $c_j=0$ \;
% }\
(Calculate $DS_{ic}$ for each phase $p_i\in\{p_1,\dots,p_P\}$ in the current signal plan)\\
\For {$i=1;i \le P;$}
{
Calculate $DS_{ic}$ using Equation~\ref{eq:scats-ds} \;
}\
(Infer $DS_{ij}$ for other signal plan)\\
\For {$j=1;j \le N$}
{
    \For {$i=1;i \le P$}
    {
       Calculate $DS_{ij} = \frac{DS_{ic}\times g_{ic}}{g_{ij}}$ \;
    }
}\
Return the signal plan $a_j$ that have the minimal $\Sigma^P_i DS_{ij}$;
\end{algorithm}


Since SCATS relies on real-time traffic detection, the cycle length, split and offset varies to adapt to change in traffic volume. However, since traffic volume is detected by loop sensors at the stop line, it is impossible to provide instantaneous feedback to traffic. That's why other signal control systems such as SCOOT implement mid-link sensors. In addition, the "adaptive" process is completed by the local controller without traffic model, which limits the use of an optimization methodology. %SCATS  over-saturation.

\paragraph{SCOOT}
SCOOT (Split Cycle Offset Optimization Technique) was first developed by Robertson's team~\cite{robertson1969tansyt} and has been extended later in several respects. It is considered to be the traffic-responsive or online version of TRANSYT, which has been applied to over 150 cities in the United Kingdom and elsewhere. 

SCOOT utilizes traffic volume and occupancy (similar to traffic density) measurements close to the entrance of links. It runs in a central control computer and employs a philosophy similar to TRANSYT. More precisely, SCOOT includes a network model that is fed with real measurements (instead of historical values) and is run repeatedly in real time to estimate the effect of a small incremental change in signal timings on the overall performance of the region's traffic signal network, which is measured through a performance index, a composite measure based on vehicle delays, and stops on each link. If the changes turn out to be beneficial, they are submitted to the local signal controllers.~\cite{luk1984two} shows through field evaluation that SCOOT's performance deteriorates in case of saturated traffic conditions.

SCOOT thus uses a coordination plan that matches the latest situation recorded as cyclic flow profiles. This is achieved by optimizing splits, offsets, and cycle time in the following way: A few seconds before every phase change, the SCOOT split optimizer makes an selection among whether it is better to advance or retard the scheduled change by up to 4 seconds, or to leave it unchanged. Then, once a cycle, the offset optimizer assesses whether the PI on streets around each junction can be reduced by altering the offset of that junction by up to 4 seconds either way. Favorable split and offset alterations are implemented immediately. In a similar way, the cycle time of a group of junctions may be incremented up or down by a few seconds every few minutes.


\paragraph{Max-pressure} The previous control systems provide poor performance under heavy traffic. Max-pressure in~\cite{varaiya2013max} minimizing the risk of over-saturation by balancing queue length between coupled intersections. The key idea of Max-pressure (MP) is to minimize the ``pressure'' of an intersection, which can be loosely defined as number of vehicles on entering lane minus the number of vehicles on exiting lane. Figure~\ref{fig:pressure} illustrates the concept of pressure. By setting the objective as minimizing the pressure of intersections, MP is proved to maximize the throughput of the whole road network~\cite{varaiya2013max}. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig/Maxpressure.pdf}
    \caption{Illustration of max pressure control in two cases. In Case A, green signal is set in the North$\rightarrow$South direction; in Case B, green signal is set in the East$\rightarrow$West direction.}
    \label{fig:pressure}
\end{figure}

At each time step, the controller calculates the pressure exerted by each phase. The pressure of a phase is defined as the sum of the weighted saturation flow rates of all movements actuated by the phase, and the weight is calculated as the difference between paired upstream and downstream queue lengths by movement. The MP controller applies green to the phase that exerts the maximum pressure each pre-defined time-step. Following store-and-forward model, it is proven that MP stabilize queuing process under feasible demand.

However, it could cause flicker of signal when two phases have similar pressure. Another concern is that traffic of minor street could sometimes wait for multiple cycles, which arises unfairness. An variant MP considers link queue storage capacity and partitions green time proportionally to phase pressures each cycle, while maintaining minimum green of each phase. This variation is applicable from an implementation point of view, however, it is impossible to provide instantaneous feedback to traffic fluctuation as the decision-making is by cycle.


\subsubsection{Optimization-based methods}
 Optimization-based methods relies on the mathematical optimization given a set of non-macroscopic inputs, including the individual intersection characteristics, the volume to capacity ratios of each intersection, the link speed, and the distance between the intersections to estimate the performance. The models make assumptions based on the inputs related to the splits and offsets to determine performance measures that can be compared to timing policies. Because the models are imperfect, a significant amount of effort is necessary to take an initially screened plan to a point that can be field implemented. The timing policies described previously, the optimization policies, and the criteria for determining which criteria to use to select a signal timing plan must be considered prior to and as a part of the optimization process. There are several basic components in these methods: objective, assumptions, and optimization approach, shown in Table~\ref{tab:optimization}.
 
\begin{table}[htb]
\caption{Optimization-based methods in transportation engineering}
\label{tab:optimization}
\begin{tabular}{c|lll}
\toprule
                                                               & \multicolumn{1}{c}{RHODES}                                                                             & \multicolumn{1}{c}{TUC}                                                                                                                                                                                                                                                                                                                          & \multicolumn{1}{c}{Max-pressure}                                                                                                                                                                              \\ \midrule
Objective                                                      & \begin{tabular}[c]{@{}l@{}}Pre-defined \\ performance index\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}Balancing the numbers of vehicles \\ within the network links\end{tabular}                                                                                                                                                                                                                                            & Maximizing pressure                                                                                                                                                                                           \\
Assumption                                                     & \begin{tabular}[c]{@{}l@{}}The traffic of next \\ cycle is identical to \\ the last cycle\end{tabular} & \begin{tabular}[c]{@{}l@{}}1. Vehicles experience constant travel\\ times along an approach and are stored\\ at the end of the link if the corresponding\\ inflow is higher than the outflow.\\ 2. The cycle time, offsets and total\\ lost time of a junction are fixed; \\ 3. The saturation flows and turning\\ rates are known.\end{tabular} & \begin{tabular}[c]{@{}l@{}}Vehicles experience constant \\ travel times along an approach \\ and are stored at the end of the \\ link if the corresponding inflow \\ is higher than the outflow.\end{tabular} \\
\begin{tabular}[c]{@{}c@{}}Optimization \\ Method\end{tabular} & Hill-climb                                                                                             & \begin{tabular}[c]{@{}l@{}}Linear programming\\ Quadratic programming\end{tabular}                                                                                                                                                                                                                                                               & Greedy      \\ \bottomrule                                                                                                                                                                                                 
\end{tabular}
\end{table}
 
%Although Max-pressure could be considered as a selection-based method, recent studies~\cite{maxpressure14} proved that max-pressure is also an optimization-based method for maximizing the throughput of the whole network.

\paragraph{RHODES}
RHODES (Real-Time Hierarchical Optimized Distributed Effective System) is a real-time traffic adaptive signal control strategy that seeks to optimize the real-time performance of a corridor or network of intersections. It extends off-line optimization of TRANSYT~\cite{robertson1969tansyt} to online version mainly based on prediction on traffic. Therefore, there are mainly two steps: prediction and incremental optimization. Prediction can be done through simply using past traffic condition assuming future traffic is similar to the past, or through traffic model that models the movement of traffic.  To provide optimal control of traffic through a network, the system:
\begin{itemize}
    \item Takes real-time input from vehicle detectors
    \item Predicts the future traffic streams throughout the network
    \item Outputs signal control settings based on these predictions
\end{itemize}


\paragraph{\textit{TUC}}
TUC relies on the store-and-forward model and optimization methods like linear programming or quadratic programming to calculate the optimal traffic signal plan for the whole network. Store-and-forward model is crucial, since it simplifies the network queue evolution process to circumvent the inclusion of discrete variables, and allows for highly efficient optimization and control methods (e.g., linear programming, quadratic programming, nonlinear programming, and multi-variable regulators) with polynomial complexity, which in turn allow even Coordinated control of large-scale networks in real time under saturated traffic conditions. 


\subsubsection{Summary of actuated control in transportation engineering}
\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item Traffic-responsive.
        %\item If suitably designed using simplified traffic models, they are potentially more efficient.
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item More costly than pre-timed and actuated methods, as they require the installation, operation, and maintenance of a real-time control system (sensors, communications, central control room, local controllers)
        \item Due to the exponential complexity of these solution algorithms, the control strategies (though conceptually applicable to a whole network) are not real-time feasible for more than one intersection presence of discrete variables that require exponential-complexity algorithms for a global minimization.
        \item Most of the methods reply on the pre-defined traffic model with constraints so as to reduce the complexity of optimization, where these model may not be static or hold in the real-world scenario.
    \end{itemize}
     
\end{itemize}

\subsection{Think out of the box: inter-region control}
All above mentioned methods are considering to optimize the traffic signal for an region, which provides detailed signal control plan for each intersection within this region. However, one of the limitation of these approaches is the sensitivity to or the dependence on the modeling accuracy. Modeling the traffic flow dynamics in urban traffic networks remains a big challenge, due to various unpredictable factors such as the route choice, time of departure, and driving behavior. Thus, former-mentioned control methods may not be able to achieve the satisfactory control performance, especially in saturated situations. 

An alternative avenue to real-time network-wide traffic signal control for urban networks is a hierarchical two-level approach, where at the first level perimeter and boundary flow control between different regions of the network advances the aggregated performance, while at the second level a more detailed control can be applied to smooth traffic movements within these regions (e.g. TUC). The macroscopic fundamental diagram (MFD) aiming at simplifying the modeling problem of traffic flow describes the evolution of network outflow and vehicle accumulation in the urban network at an aggregate level. It provides for network regions under specific regularity conditions (mainly homogeneity in the spatial distribution of congestion and the network topology), a unimodal, low-scatter relationship between network vehicle accumulations n (veh) and network outflow (veh/h), as shown in Figure~\ref{fig:diagram}.



As is shown in Figure~\ref{fig:diagram}, the critical accumulation corresponding to the maximum outflow $Q_{max}$ and the span $n_1 \sim n_2$ represents the range of vehicle accumulations which can produce almost the same maximum outflow around the critical accumulation $\tilde{n}$. 
In Figure~\ref{fig:diagram}, the region $L_1$ reflects that the traffic states are undersaturated; that is, the green times are partially wasted due to lack of sufficient traffic demand. Traffic states along the line $L_2$ indicate that the traffic flows are partially saturated; that is, most links in the network experience saturated traffic flow during respective green times without obvious queue
spillback to upstream intersections. The traffic states on the declining line $L_3$ imply that there are significant queue spillbacks in some links and several upstream intersections are blocked, where the green times are seriously wasted. The growth of the vehicles number within this region will  remarkably decrease the network outflow. Finally, region $L_4$ denotes that a complete network-wide gridlock takes place, where the network outflow nearly equals zero. Once this situation occurs, any signal control strategy may be powerless.

Note that the slope of line $L_1$ indicates the average speed of vehicles in the networks. This average speed may be increased via proper traffic signal operations and a larger maximum network outflow $Q'_{max}$ max with wider vehicle accumulation span $n'_1  \sim n'_2$ can be obtained (as indicated by dotted line in Figure~\ref{fig:diagram}). The over-saturated traffic conditions (region $L_3$) can also be ameliorated by better adapted control strategies.

\cite{daganzo2007urban,keyvan2012exploiting,geroliminis2013optimal} proposed perimeter flow control policies to improve mobility in homogeneous networks. The general idea of a perimeter flow control policy is to ``meter'' the input flow to the system and to hold vehicles outside the controlled area if necessary. \cite{daganzo2007urban} used the MFD concept to propose a control rule that maximizes the network outflow; however, as discussed in \cite{keyvan2012exploiting}, the rule cannot be directly employed for practical use in urban networks. Other works~\cite{geroliminis2013optimal, strating2010coordinated} pursued a model-predictive control (MPC) approach. However, MPC calls for sufficiently accurate model and external disturbance predictions, which may be a serious impediment for practicable.
control.

A feedback-based gating concept was introduced in ~\cite{keyvan2012exploiting}, where the urban MFD was exploited to derive a simple control design model and a corresponding feedback control structure, suitable for smooth and efficient operations. The feedback concept targets an operating MFD point of maximum throughput and was demonstrated, within a realistic microscopic simulation environment, to enable sensible improvements in case of over-saturation, when fed with real-time measurements from all links of the network to be protected. \cite{aboudolas2013perimeter} extended the feedback approach for application to multiple networks with separate individual MFDs. This approach may prove beneficial in cases of big congested networks with strong inhomogeneity ~\cite{geroliminis2011properties}.

\subsubsection{Summary of inter-region control}
\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item It does not require high computational effort if proxies for critical vehicle accumulation $\tilde{n}$ are available (e.g. critical accumulation, critical average occupancy or critical density) and the current state of the network can be observed with loop detector data in real-time.

    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item  it creates queues blocking the urban roads outside the controlled area. 
        \item It does not provide traffic signal plan for all intersections in the region, which may lead to instant congestion for inner intersections.
    \end{itemize}
     
\end{itemize}

\nop{

Max-pressure in~\cite{varaiya2013max} can be utilized in traffic signal networks.

\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item requires only local information: the phase duration selected at any intersection depends only on queues adjacent to that intersection
        \item max-pressure is provably stable: it stabilizes a demand whenever there exists any stabilizing controller.
        \item max-pressure requires no knowledge of the demand, although it needs turn ratios provably maximizes throughput
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item 
        \item 
    \end{itemize}
     
\end{itemize}



\subsection{Coordinated intersection control for over-saturated networks}
An over-saturated traffic environment is fundamentally different from an understaturated environment. In undersaturated networks, capacity is adequate and queue lengths are generally well contained within individual approaches. The over-saturated environment is characterized by an excess of demand relative to capacity ($v/c > 1.0$) and thus unstable queues that tend to expand over time with the potential of physically blocking intersections (blockage, spillback), thus slowing queue discharge rates and, in effect, reducing capacity when it is most needed. Control policies for over-saturated networks therefore focus on maintaining and fully exploiting capacity to maximize productivity (vehicle throughput) of the system by controlling the inherent instability of queue growth.


\subsubsection{Strategies}
\begin{itemize}
    \item Internal metering: the use of control strategies within a congested network so as to influence the distribution of vehicles arriving or departing from a critical location.
    \item External metering: Control of the major access points to the target system so that inflow rates into the system are limited if the system is already too congested.
\end{itemize}


\subsection{Classical systems}

\begin{table}[]
\begin{tabular}{lllllll}
& Action  & Adjustment & Time Frame & Level                                                        & \begin{tabular}[c]{@{}l@{}}Traffic \\ Modeling\end{tabular} & \begin{tabular}[c]{@{}l@{}}Type of \\ adjustment\end{tabular} \\
ACSLite & P \& R     & RBA        & 5-10 min                                                     & Hierachical                                                 & No                                                            & S, O         \\
UTCS-1  & P \& R     & OBA        & 5 min                                                        & Hierachical                                                 & Yes                                                           & S, Cl, O,PS  \\
LA ATCS & P \& R     & RBA,OBA    & Cycle                                                        & Hierachical                                                 & Yes                                                           & S, Cl, O     \\
OPAC    & P          & OBA        & \begin{tabular}[c]{@{}l@{}}Phase/Cycle\\ /5 min\end{tabular} & Hierachical                                                 & Yes                                                           & S, Cl, O     \\
RHODES  & P          & OBA        & Sec by sec                                                   & Hierachical                                                 & Yes                                                           & S            \\
SCATS   & R          & RBA        & Cycle                                                        & Hierachical                                                 & No                                                            & S, Cl, O     \\
SCOOT   & P \& R     & OBA        & Cycle/5 min                                                  & Hierachical                                                 & Yes                                                           & S, Cl, O, PS \\
UTOPIA  & P          & OBA        & 3 sec - Cycle                                                & Hierachical                                                 & Yes                                                           & S, PS       
\end{tabular}
\end{table}


\subparagraph{Methods and systems}
McShane, Traffic engineering, 1990.
Cools, Self-organizing traffic lights: A realistic simulation 2013



\subsubsection{1st Generation}
These methods use libraries of signal control plans which are trained off-line and selected by operators or time triggers. Control plans are usually designed on historical data for different periods of time (e.g., time of day, day of week).

\subparagraph{Pros}
Simple and straightforward operation
Suitable for relatively predictable traffic flow
Can be updated after long periods of time (usually updated every 2 to 10 years)

\subparagraph{Cons}
Cannot efficiently handle long-term non-stationary traffic flow (e.g., stochastic variations in traffic patterns, non-recurrent traffic congestion)
Need to store traffic flows in advance and then update manually


\subsubsection{2nd Generation}
These methods use online optimization methods to dynamically adjust signal timings with the help of surveillance facilities (e.g., loop sensors). Though centralized controlling over system performance, 2nd generation methods update their control strategies if there is possible improvement after the update for next cycle. 
\subparagraph{Systems}
SCATS and SCOOTS.

\subparagraph{Pros}
Responsive to random fluctuation in traffic demand. 

\subparagraph{Cons}
Limited closed loop optimal control and coordination abilities.
Centralized control may relies on reliable networks.
Not scalable to large network.
Expensive for installation and maintenance.


\subsubsection{3rd Generation}
Similar to the 2-GC systems, 3rd generation systems and methods can adapt to traffic fluctuations but operate in a decentralized fashion.
Most methods use dynamic programming techniques to model and solve the decentralized traffic signal control problem, which captures the stochastic nature and dynamics of the traffic system.
\subparagraph{Systems}
OPAC (Gartner, 1983)

PRODYN (Farges et al., 1983). local controller gives original decision, sent this decision to supervisor;
supervisor calculate the possible state change according to local decisions, and sent back these info;
local controller update the decision with new info, sent back to supervisor;
if solution doesn't change, keep it; else recompute.

UTOPIA/SPOT (Mauro and Di Taranto, 1989a)

RHODES (Head et al., 1992). Predict traffic flow first, explicitly set phases that maximize a given traffic performance measure using DP.


\subparagraph{Pros}
less computationally less expensive as only require and maintain the relevant information from the surrounding intersections.
more robust to temporary breakdowns of individual intersections.
more flexible in cycle length.

\subparagraph{Cons}
The performances of methods largely rely on the prediction on traffic flow.
Solving DP algorithms with Webster-like methods are delicately designed, computationally intractable (Sutton and Barto, 1998; Gosavi, 2003) which hinders a straightforward network-wide application of the optimization method. 

\subsubsection{4th Generation}
self-learning approaches that are based on experience under real-time conditions. 
\subparagraph{Systems}
\subparagraph{Pros}
\subparagraph{Cons}
some of the previous studies were primarily conducted to either control an isolated traffic element or multiple controller, but with no action coordination between the traffic controllers. (Abdulhai et al., 2003; Bakker et al., 2005; Camponogara and Kraus Jr., 2003; De Oliveira et al., 2006; Thorpe, 1997; Wiering, 2000) the agents may select individual actions that are locally optimal but suboptimal solutions for the network (Busoniu et al., 2008)

Coordination using max-plus algorithm is computationally expensive as it requires negotiations between the agents to coordinate their actions through direct communication.

}


% Specifically, at each time step, the controller calculates the pressure exerted by each phase. The pressure of a phase is defined as the sum of the weighted saturation flow rates of all movements actuated by the phase, and the weight is calculated as the difference between paired upstream and downstream queue lengths by movement. The MP controller applies green to the phase that exerts the maximum pressure each pre-defined time-step. Following store-and-forward model, it is proven that MP stabilize queuing process under feasible demand.

%However, this approach have serveral drawbacks: a) when the control cycle is large, queues can grow unexpectedly in traffic movements that are not activated. However, it could cause flicker of signal when two phases have similar pressure. %Another concern is that traffic of minor street could sometimes wait for multiple cycles, which arises unfairness. An variant \Maxpressure considers link queue storage capacity and partitions green time proportionally to phase pressures each cycle, while maintaining minimum green of each phase. This variation is applicable from an implementation point of view, however, it is impossible to provide instantaneous feedback to traffic fluctuation as the decision-making is by cycle.

%  \paragraph{\textit{TUC}}
% TUC relies on the store-and-forward model and optimization methods like linear programming or quadratic programming to calculate the optimal traffic signal plan for the whole network. Store-and-forward model is crucial, since it simplifies the network queue evolution process to circumvent the inclusion of discrete variables, and allows for highly efficient optimization and control methods (e.g., linear programming, quadratic programming, nonlinear programming, and multi-variable regulators) with polynomial complexity, which in turn allow even Coordinated control of large-scale networks in real time under saturated traffic conditions. 

 


    %Isolated vs. coordinated control. Modern urban traffic-control system is not only just signal plan of intersections, but also signal coordination of a large traffic networks, which includes arterial and grid-like regions. Coordination is largely a strategic approach to synchronize signals together to meet specific objectives. While there are numerous objectives for the coordination of traffic signals, common objectives are stated succinctly in ~\cite{koonce2008traffic}: The intent of coordinating traffic signals is to provide smooth flow of traffic along streets and highways in order to reduce travel times, stops and delay, which reduces fuel consumption and improves air quality. Various performance measures can be used to evaluate signal coordination. Isolated intersection performance measures include delay, queue length, and safety; however, performance measures for coordinated systems may be slightly different. Evaluation methods include the number of stops reduced for the main street through movements or queue management. With the modern signal controller, coordination is accomplished by adding a layer of logic (that is, coordination logic compliments some basic features such as when a phase can begin or end) to the basic actuated logic used for isolated signal timing operations. In previous sections, the details of the controller settings were limited to those applied at isolated or independent intersections (cycle length, phase split, maximum green, pedestrian timing, etc).
    

 
%  \subsubsection{Division of search space}
% Division of search space indicates the method optimizes the traffic signal plans in two steps: \textit{Step 1}: optimize for a single intersection by adjusting the cycle length and phase split; \textit{Step 2}: adjusting offsets for multiple intersections.
 
 \begin{table}[htb]
\caption{Optimization-based methods with the division of search space in transportation engineering}
\label{tab:two-step}
\begin{tabular}{p{3cm} p{3cm} p{6cm} p{2cm}}
\toprule
            & Objective    & Assumption    & Approach      \\ \midrule
\Formula (single intersection) & Minimize duration & uniform traffic   & Close-form solution \\ \hline
\Greenwave  & Minimize duration for traffic along one certain direction & 
\begin{tabular}[c]{@{}l@{}}
1. uniform traffic, \\ 
2. no turning, \\ 
3. identical traffic for all intersections \\ 
4. no digestion on traffic\\ 
5. the vehicles travel with given speed\\ and the distance between intersection\\ are known in advance.\end{tabular} & Close-form  solution \\ \hline
\Maxband     & Maximize the bandwidth for two directions & uniform traffic   & Linear programming \\ \bottomrule
\end{tabular}
\end{table}


==> deleted.tex <==
\subsubsection{Pre-timed control}
In pre-timed control, the cycle length, phase sequence and time of each phase are constant. In field operations, adjustments could be done through a fixed signal plan for the entire day, or variability throughout the day, e.g., different fixed signal plan during AM or PM peak period and off-peak period.


\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item Computationally efficient.
        \item Effective in networks with well-behaved traffic patterns, i.e., the traffic patterns are very similar over different time periods.
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item The signal plans are computed for a static situation, based on historical data. It is known that nowadays demand may not be constant, neither between days, nor during the day, nor in a given traffic direction. The operation of networks close to the saturation flow increases the chances of accidents which, in turn, contribute to unexpected patterns.
        \item Even if the computation itself is not manual, this is a complex task that requires a lot of expert knowledge as well as historical data. 
        \item Unsuitable for dynamic or unexpected traffic conditions. 
    \end{itemize}
\end{itemize}


\subsection{Vehicle-actuated control}
In vehicle-actuated control, the actuation by a vehicle on one or more approaching lanes is required for certain phases or traffic movements to be serviced based on certain rules. When the time gap between detector activations (the detector is activated whenever a vehicle passes) exceeds some pre-defined threshold, current phase terminates~\cite{RPM04}. In field operations, there are three basic types of this method, different in the rules utilized: call-based-actuation control and volume-density control.



\subsection{Think out of the box: inter-region control}
All above mentioned methods are considering to optimize the traffic signal for an region, which provides detailed signal control plan for each intersection within this region. However, one of the limitation of these approaches is the sensitivity to or the dependence on the modeling accuracy. Modeling the traffic flow dynamics in urban traffic networks remains a big challenge, due to various unpredictable factors such as the route choice, time of departure, and driving behavior. Thus, former-mentioned control methods may not be able to achieve the satisfactory control performance, especially in saturated situations. 

An alternative avenue to real-time network-wide traffic signal control for urban networks is a hierarchical two-level approach, where at the first level perimeter and boundary flow control between different regions of the network advances the aggregated performance, while at the second level a more detailed control can be applied to smooth traffic movements within these regions (e.g. TUC). The macroscopic fundamental diagram (MFD) aiming at simplifying the modeling problem of traffic flow describes the evolution of network outflow and vehicle accumulation in the urban network at an aggregate level. It provides for network regions under specific regularity conditions (mainly homogeneity in the spatial distribution of congestion and the network topology), a unimodal, low-scatter relationship between network vehicle accumulations n (veh) and network outflow (veh/h), as shown in Figure~\ref{fig:diagram}.


As is shown in Figure~\ref{fig:diagram}, the critical accumulation corresponding to the maximum outflow $Q_{max}$ and the span $n_1 \sim n_2$ represents the range of vehicle accumulations which can produce almost the same maximum outflow around the critical accumulation $\tilde{n}$. 
In Figure~\ref{fig:diagram}, the region $L_1$ reflects that the traffic states are undersaturated; that is, the green times are partially wasted due to lack of sufficient traffic demand. Traffic states along the line $L_2$ indicate that the traffic flows are partially saturated; that is, most links in the network experience saturated traffic flow during respective green times without obvious queue
spillback to upstream intersections. The traffic states on the declining line $L_3$ imply that there are significant queue spillbacks in some links and several upstream intersections are blocked, where the green times are seriously wasted. The growth of the vehicles number within this region will  remarkably decrease the network outflow. Finally, region $L_4$ denotes that a complete network-wide gridlock takes place, where the network outflow nearly equals zero. Once this situation occurs, any signal control strategy may be powerless.

Note that the slope of line $L_1$ indicates the average speed of vehicles in the networks. This average speed may be increased via proper traffic signal operations and a larger maximum network outflow $Q'_{max}$ max with wider vehicle accumulation span $n'_1  \sim n'_2$ can be obtained (as indicated by dotted line in Figure~\ref{fig:diagram}). The over-saturated traffic conditions (region $L_3$) can also be ameliorated by better adapted control strategies.

\cite{daganzo2007urban,keyvan2012exploiting,geroliminis2013optimal} proposed perimeter flow control policies to improve mobility in homogeneous networks. The general idea of a perimeter flow control policy is to ``meter'' the input flow to the system and to hold vehicles outside the controlled area if necessary. \cite{daganzo2007urban} used the MFD concept to propose a control rule that maximizes the network outflow; however, as discussed in \cite{keyvan2012exploiting}, the rule cannot be directly employed for practical use in urban networks. Other works~\cite{geroliminis2013optimal, strating2010coordinated} pursued a model-predictive control (MPC) approach. However, MPC calls for sufficiently accurate model and external disturbance predictions, which may be a serious impediment for practicable.
control.

A feedback-based gating concept was introduced in ~\cite{keyvan2012exploiting}, where the urban MFD was exploited to derive a simple control design model and a corresponding feedback control structure, suitable for smooth and efficient operations. The feedback concept targets an operating MFD point of maximum throughput and was demonstrated, within a realistic microscopic simulation environment, to enable sensible improvements in case of over-saturation, when fed with real-time measurements from all links of the network to be protected. \cite{aboudolas2013perimeter} extended the feedback approach for application to multiple networks with separate individual MFDs. This approach may prove beneficial in cases of big congested networks with strong inhomogeneity ~\cite{geroliminis2011properties}.

\subsubsection{Summary of inter-region control}
\paragraph{Pros and Cons}
\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item It does not require high computational effort if proxies for critical vehicle accumulation $\tilde{n}$ are available (e.g. critical accumulation, critical average occupancy or critical density) and the current state of the network can be observed with loop detector data in real-time.

    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item  it creates queues blocking the urban roads outside the controlled area. 
        \item It does not provide traffic signal plan for all intersections in the region, which may lead to instant congestion for inner intersections.
    \end{itemize}
     
\end{itemize}

\nop{

\Maxpressure  in~\cite{varaiya2013max} can be utilized in traffic signal networks.

\begin{itemize}
    \item Pros. 
    \begin{itemize}
        \item It requires only local information: the phase duration selected at any intersection depends only on queues adjacent to that intersection
        \item It is provably stable: it stabilizes a demand whenever there exists any stabilizing controller.
        \item It requires no knowledge of the demand, although it needs turn ratios provably maximizes throughput
    \end{itemize}
    \item Cons.
    \begin{itemize}
        \item 
        \item 
    \end{itemize}
     
\end{itemize}



\subsection{Coordinated intersection control for over-saturated networks}
An over-saturated traffic environment is fundamentally different from an understaturated environment. In undersaturated networks, capacity is adequate and queue lengths are generally well contained within individual approaches. The over-saturated environment is characterized by an excess of demand relative to capacity ($v/c > 1.0$) and thus unstable queues that tend to expand over time with the potential of physically blocking intersections (blockage, spillback), thus slowing queue discharge rates and, in effect, reducing capacity when it is most needed. Control policies for over-saturated networks therefore focus on maintaining and fully exploiting capacity to maximize productivity (vehicle throughput) of the system by controlling the inherent instability of queue growth.


\subsubsection{Strategies}
\begin{itemize}
    \item Internal metering: the use of control strategies within a congested network so as to influence the distribution of vehicles arriving or departing from a critical location.
    \item External metering: Control of the major access points to the target system so that inflow rates into the system are limited if the system is already too congested.
\end{itemize}


\subsection{Classical systems}

\begin{table}[]
\begin{tabular}{lllllll}
& Action  & Adjustment & Time Frame & Level                                                        & \begin{tabular}[c]{@{}l@{}}Traffic \\ Modeling\end{tabular} & \begin{tabular}[c]{@{}l@{}}Type of \\ adjustment\end{tabular} \\
ACSLite & P \& R     & RBA        & 5-10 min                                                     & Hierachical                                                 & No                                                            & S, O         \\
UTCS-1  & P \& R     & OBA        & 5 min                                                        & Hierachical                                                 & Yes                                                           & S, Cl, O,PS  \\
LA ATCS & P \& R     & RBA,OBA    & Cycle                                                        & Hierachical                                                 & Yes                                                           & S, Cl, O     \\
OPAC    & P          & OBA        & \begin{tabular}[c]{@{}l@{}}Phase/Cycle\\ /5 min\end{tabular} & Hierachical                                                 & Yes                                                           & S, Cl, O     \\
RHODES  & P          & OBA        & Sec by sec                                                   & Hierachical                                                 & Yes                                                           & S            \\
SCATS   & R          & RBA        & Cycle                                                        & Hierachical                                                 & No                                                            & S, Cl, O     \\
SCOOT   & P \& R     & OBA        & Cycle/5 min                                                  & Hierachical                                                 & Yes                                                           & S, Cl, O, PS \\
UTOPIA  & P          & OBA        & 3 sec - Cycle                                                & Hierachical                                                 & Yes                                                           & S, PS       
\end{tabular}
\end{table}


\subparagraph{Methods and systems}
McShane, Traffic engineering, 1990.
Cools, Self-organizing traffic lights: A realistic simulation 2013



\subsubsection{1st Generation}
These methods use libraries of signal control plans which are trained off-line and selected by operators or time triggers. Control plans are usually designed on historical data for different periods of time (e.g., time of day, day of week).

\subparagraph{Pros}
Simple and straightforward operation
Suitable for relatively predictable traffic flow
Can be updated after long periods of time (usually updated every 2 to 10 years)

\subparagraph{Cons}
Cannot efficiently handle long-term non-stationary traffic flow (e.g., stochastic variations in traffic patterns, non-recurrent traffic congestion)
Need to store traffic flows in advance and then update manually


\subsubsection{2nd Generation}
These methods use online optimization methods to dynamically adjust signal timings with the help of surveillance facilities (e.g., loop sensors). Though centralized controlling over system performance, 2nd generation methods update their control strategies if there is possible improvement after the update for next cycle. 
\subparagraph{Systems}
SCATS and SCOOTS.

\subparagraph{Pros}
Responsive to random fluctuation in traffic demand. 

\subparagraph{Cons}
Limited closed loop optimal control and coordination abilities.
Centralized control may relies on reliable networks.
Not scalable to large network.
Expensive for installation and maintenance.


\subsubsection{3rd Generation}
Similar to the 2-GC systems, 3rd generation systems and methods can adapt to traffic fluctuations but operate in a decentralized fashion.
Most methods use dynamic programming techniques to model and solve the decentralized traffic signal control problem, which captures the stochastic nature and dynamics of the traffic system.
\subparagraph{Systems}
OPAC (Gartner, 1983)

PRODYN (Farges et al., 1983). local controller gives original decision, sent this decision to supervisor;
supervisor calculate the possible state change according to local decisions, and sent back these info;
local controller update the decision with new info, sent back to supervisor;
if solution doesn't change, keep it; else recompute.

UTOPIA/SPOT (Mauro and Di Taranto, 1989a)

RHODES (Head et al., 1992). Predict traffic flow first, explicitly set phases that maximize a given traffic performance measure using DP.


\subparagraph{Pros}
less computationally less expensive as only require and maintain the relevant information from the surrounding intersections.
more robust to temporary breakdowns of individual intersections.
more flexible in cycle length.

\subparagraph{Cons}
The performances of methods largely rely on the prediction on traffic flow.
Solving DP algorithms with Webster-like methods are delicately designed, computationally intractable (Sutton and Barto, 1998; Gosavi, 2003) which hinders a straightforward network-wide application of the optimization method. 

\subsubsection{4th Generation}
self-learning approaches that are based on experience under real-time conditions. 
\subparagraph{Systems}
\subparagraph{Pros}
\subparagraph{Cons}
some of the previous studies were primarily conducted to either control an isolated traffic element or multiple controller, but with no action coordination between the traffic controllers. (Abdulhai et al., 2003; Bakker et al., 2005; Camponogara and Kraus Jr., 2003; De Oliveira et al., 2006; Thorpe, 1997; Wiering, 2000) the agents may select individual actions that are locally optimal but suboptimal solutions for the network (Busoniu et al., 2008)

Coordination using max-plus algorithm is computationally expensive as it requires negotiations between the agents to coordinate their actions through direct communication.

}




--------2019.03.21---------


\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\columnwidth]{fig/phase.png}
\caption{Definitions of traffic movement and traffic signal phases.}
\label{fig:phase}
\end{figure}

\section{Preliminary}
\label{sec:basic-tlcs}
\subsection{Term Definition}


Terms on road structure and traffic movement:
\begin{itemize}
    \item \textbf{Road}: For an intersection, there are two kinds of roads: the approaching road and the receiving road. An approaching road is where a car enters an intersection; a receiving road is where a car leaves an intersection. Figure~\ref{fig:phase}(a) shows a typical intersection with twelve approaching roads and receiving roads, where we point out the North approaching road.  
    \item \textbf{Lane}: A road consists of a set of lanes. Corresponding to road, there are two kinds of lanes: the approaching lane and the receiving lane.
    \item \textbf{Traffic movement}: A traffic movement is generally categorized as left turn, through, and right turn. A road-level traffic movement means the vehicles moving from an approaching road to a receiving road. A signal-level traffic movement aggregates the road-level traffic movements controlled by the same traffic signal. For example, if there are multiple through traffic lanes, they belong to the same road-level traffic movement; if the through traffic and the left-turn traffic movement are controlled by one signal, they belong to the same signal-level traffic movement.
   % In Figure~\ref{fig:phase}(a), we show that there are $8$ traffic movements. Follow the traffic rules in most countries, right turn traffic can pass regardless of the signal, but it needs to yield on a red light. 

\end{itemize}

Terms on traffic signal:
\begin{itemize}
    \item \textbf{Movement signal}: For each signal-level traffic movement, we can use one bit with 1 as `green' signal and 0 as `red'. Commonly when the right-turn traffic can pass regardless of the signal, there are eight movement signals in use, as shown in Figure~\ref{fig:phase}(b).   
    \item \textbf{Phase}:  A phase is a combination of movement signals. %Usually the combination of movement signals should avoid the conflict between traffic movements, i.e., when the green light is on for those movements, the vehicles in one movement do not necessarily yield to the vehicles from other movements to avoid collision. 
    As indicated by the conflict matrix in Figure~\ref{fig:phase}(c), some signals cannot turn `green' at the same time (e.g., signals \#1 and \#2) so that the vehicles in one movement do not necessarily yield to the vehicles from other movements to avoid the collision. All the non-conflicting signals will generate eight valid paired-signal phases (letters `A' to 'H' in Figure~\ref{fig:phase}(c)) and eight single-signal phases (the diagonal cells in conflict matrix). %Here we do not consider the single-signal phase  because in an isolated intersection, it is always more efficient to use paired-signal phases. 
    \item \textbf{Phase sequence}:  A phase sequence is a sequence of phases which defines a set of phases and their order of changes.
    \item \textbf{Cycle}: A cycle consists of a sequence of phases and their corresponding temporal duration. For example, in a 180-second cycle, we can define 100-second phase $A$ and 80-second phase $E$. Existing traffic signal control system usually repeats similar cycles throughout the day.  

    %\item Offset. The time relationship, expressed in either seconds or as a percent of the cycle length, between coordinated phases at subsequent traffic signals. The offset is dependent on the offset reference point, which is defined as that point within a cycle in which the local controller's offset is measured relative to the master clock. It is not necessarily the same as the deterministic point (or yield point) within the cycle. 
    %\item Total Lost Time ($tL_i$) - Time during which the intersection is not effectively used by any movement.
    %\item Coordination. The ability to synchronize multiple intersections to enhance the operation of one or more directional movements in a system.
\end{itemize}



\subsection{Objective}
The objective of traffic signal control is to facilitate more efficient transportation. Different measures have been proposed to quantify this objective from different perspectives: 
\begin{itemize}
    \item Travel time. In traffic signal control, one of the most common goals is to minimize the average travel time of vehicles in the network: by minimizing travel time, congestion is indirectly discouraged and traffic throughput optimized. However, the travel time of a vehicle is unknown until it has reached its destination. 
    % \item Average delay per vehicle. Delay measures the excess time consumed in traversing the intersection \textcolor{red}{jessie: broken sentence}
    \item Queue length. The queue length of the system is the number of vehicles that have entered the system but are still waiting to leave the network. 
    \item Number of stops. The umber of stops of a vehicle is the total times that a vehicle experienced. For a traffic signal control system, the average number of stops over all vehicles in the system is especially important where the increase in the number of stops will lead to more emission. 
    \item System throughput. The throughput of a system is the number of vehicles that have reached their destination or left the system during throughout a period. Maximizing throughput is the primary objective when the system is congested. % which can be achieved by (a) avoiding queue spillback, which blocks intersections and wastes green time; (b) avoiding tardy arrival of traffic; and (c) managing queue formation to yield the highest service across the stop line.
    % \item Fully utilize storage capacity.  This objective seeks to confine the congestion to a limited area by managing queue formation.
    %\item Provide equitable service. This seeks to allocate service to cross traffic and to left-turners so that all travelers are serviced adequately.
\end{itemize}

\subsection{Special considerations}
In practice, additional attention should be paid to the following aspects:
 
\begin{enumerate}
\item Yellow and all-red signal. This allows vehicles to stop safely or pass the intersection before vehicles in conflicting traffic movements are given a green signal.

\item Minimum green time. Usually, a minimum green signal time is required to ensure the pedestrian can pass through the intersection.

\item Left turn phase. Usually, a left-turn phase is added when the left-turn flow is above a manually designed threshold.

\end{enumerate}



\nop{
\begin{figure}[t]
  \centering
  \begin{tabular}{cc}
   \includegraphics[width=0.42\textwidth]{fig/Time-Space-Diagram.png} & 
   \includegraphics[width=0.48\textwidth]{fig/MFD.png}
   \end{tabular}
   \vspace{-1mm}
     \caption{Space-time diagram and Macroscopic fundamental diagram.}
\label{fig:diagram}
\end{figure}
}




\nop{

    %\item Interval. Period of Time during which all signal indications remain constant. 
    %\item Green Interval ($G_i$) - Green indication (sec).
    %\item Red Interval ($R_i$) - Red indication (sec).
    %\item Clearance/All red Interval ($ar_i$) - all movements have red signal (sec).
    %\item Change Interval ($y_i$) - the yellow indication for a given movement (sec).
    %\item Effective Green Time ($g_i$) = $G_i+ y_i + ar_i - tL_i$
    %\item Effective Red Time ($r_i$) = $C - G_i$
    
    
    
   % \item Time-Space Diagram. A chart that plots the location of signalized intersections along the vertical axis and the signal timing along the horizontal axis. This is a visual tool that illustrates coordination relationships between intersections.
    %\item Bandwidth. Bandwidth is described as the amount of time available for vehicles to travel through an arterial at a determined progression speed. This is an outcome of the signal timing that is determined by the offsets between intersections and the allotted green time for the coordinated phase at each intersection. The bandwidth is calculated by the difference between the first and last vehicle trajectory that can travel at the progression speed without impedance. Bandwidth is a parameter that is commonly used to describe capacity or maximize vehicle throughput, but in reality it is only a measure of progression opportunities. Bandwidth is independent of traffic flows and travel paths and for that reason it may not necessarily be used by travelers. 
    %\item Macroscopic Fundamental Diagram (MFD).  The MFD of urban traffic defines a unimodal low-scatter relationship between network outflow and network vehicle accumulation for a homogeneous network. It is observed that the maximum outflow of the network may be over a range of vehicle accumulation values that is close to a critical accumulation. The typical shape of an MFD for urban networks is shown in Figure~\ref{fig:diagram}.
}
